Imagerie des \'etoiles \'evolu\'ees par interf\'erom\'etrie. R\'earrangement de pupille

Atmospheric turbulence is an important limit to high angular resolution in astronomy. Interferometry resolved this issue by filtering the incoming light with single-mode fibers. Thanks to this technique, we obtained with the IOTA interferometer very precise measurements of the spatial frequencies of seven evolved stars. From these measurements, we performed a blind deconvolution to restore an image of the surface of the stars. Six of the them, Betelgeuse, Mu Cep, R leo, Mira, Chi Cyg and CH Cyg, feature very asymmetrical brightness distributions. On the other hand, the Arcturus data are extremely well fitted with a simple limb-darkened photospheric disc. From the observations of $\chi$ Cyg, we show that the star is surrounded by a molecular shell undergoing a ballistic motion. We propose to use the same technique of spatial filtering with single-mode fibers to correct for the effect of turbulence in the pupil of a telescope. Because the pupil is redundant, this technique does require a remapping of the pupil. We developed a dedicated algorithm to show that it was possible to reconstruct images at the diffraction limit of the telescope free of any speckle noise. Our simulations show that a high dynamic range (over 10^6) could be obtained in the visible on an 8 meter telescope. A lab experiment is under construction to validate the concept of this new instrument.

==> etoile3.tex <==
\newpage

\section{Les étoiles évoluées}

\subsection{La formation d'étoiles géantes}


Une étoile est une boule de gaz maintenant un équilibre (stable ou
instable) entre force gravitationnelle et pression interne. Cette
dernière peut être radiative, thermique ou encore due à un gaz de
particules relativistes. Au sein de la séquence principale, la force
de pression est maintenue par la fusion de la matière contenue dans le
c\oe ur de l'étoile. C'est le cas de tout astre ayant une masse
supérieure à 0,08 M$_\odot$ (nécessaire pour permettre la fusion de
l'hydrogène) et inférieure à 100 M$_\odot$ (limite supérieure à partir de
laquelle la pression est tellement grande qu'elle engendre
l'instabilité de l'étoile). Parce qu'il s'agit justement de résister à
la pression gravitationnelle, les étoiles consomment de l'énergie. Le
``carburant'' étant nécessairement une ressource finie, il est logique
que les étoiles aient une certaine durée de vie. Elles ont été créées à
un moment précis, et s'éteindront lorsque leurs sources d'énergie
s'épuiseront. Il s'en déduit la notion d'évolution stellaire.

L'étoile naît d'un nuage de gaz auto-gravitant qui se contracte sous
l'effet de la gravitation. L'énergie potentielle gravitationnelle est
alors libérée sous forme de chaleur permettant, à terme, la fusion de
l'hydrogène (dés que la température interne atteint $\approx 10^7$ K)
qui est le premier combustible nucléaire à être utilisé par les
étoiles. S'ensuit la possible fusion de l'Hélium, du Carbone, du Néon,
de l'Oxygène, du Silicium, et plus généralement de toutes les espèces
d'indices atomiques inférieurs à celui du Fer.

En conséquence, l'évolution stellaire peut être résumée comme
suit. Durant une première phase d'évolution se forme une boule
homogène constituée principalement d'hydrogène. La transformation de
cet élément (composant A) en un composant B (Hélium), produit de
l'énergie nucléaire. Quand l'élément A est épuisé au c\oe ur de
l'étoile, la source d'énergie s'arrête, et le gradient de pression
disparaît. Le c\oe ur est alors composé de l'élément B, entouré d'une
enveloppe constituée principalement de l'élément A. Sous l'effet de sa
propre gravité, le c\oe ur se contracte et sa température
augmente. Parallèlement, l'enveloppe se dilate, et se refroidit
(Théorème du viriel). Il se peut alors que l'augmentation de la
température à la surface du c\oe ur permette la fusion en couche de A
en B, augmentant ainsi la masse du c\oe ur et sa vitesse
d'effondrement. Si la température du c\oe ur atteint un niveau
suffisant, l'élément B peut fusionner, créant une nouvelle source
d'énergie. La contraction du c\oe ur s'arrête alors, et B est
transformé en C. L'étoile se compose des éléments C, B et A répartis
respectivement dans différentes couches allant du c\oe ur à la surface
de l'étoile. Ce phénomène se répète pour des élément D, E, F, de
masses atomiques toujours plus grandes (Carbone, Néon, Oxygène, ...),
avec toujours une stratification de l'étoile et une augmentation de la
taille de l'enveloppe stellaire.


\subsection{L'évaporation des étoiles}

\begin{figure} 
\centering 
\resizebox{\hsize}{!}{\includegraphics{Images/87_204.eps}}
   \caption{ Nébuleuse de la Lyre (M57), une nébuleuse planétaire qui
   était autrefois une géante rouge. Le coeur et l'enveloppe de
   poussière sont devenus respectivement une naine blanche et un
   anneau de poussières entourant celle-ci. Crédit: W. M. Keck Observatory }
   \label{fig:M57} 
\end{figure}

L'évolution d'une galaxie dépend principalement de la matière qui la
compose. Fruit de la nucléosynthèse primordiale, la matière originelle
est principalement composée d'Hydrogène, de Deutérium et de Lithium. \`A
partir de cette matière, des étoiles se forment, au c\oe ur desquelles
des éléments plus lourd se créent. Ces éléments sont ensuite relâchés
dans le milieu interstellaire, et participent à la formation d'une
nouvelle population d'étoiles. On note, par exemple, la coexistence
dans notre galaxie de deux populations (Population I et II)
qui se caractérisent par une proportion de métaux (tout élément de
masse atomique supérieure à l'Helium) différente. Ce phénomène, appelé
l'astration, dépend en grande partie de la capacité des étoiles à
rejeter la matière modifiée en leur c\oe ur dans le milieu
interstellaire. La maîtrise de ce processus est fondamentale à la
compréhension de l'évolution galactique. Le rejet de matières s'opère
de deux manières:
\begin{itemize}
\item Novae et Supernovae: il s'agit d'un phénomène relativiste qui se 
caractérise par une éjection massive et rapide des couches
superficielles de l'étoile. Ce taux de rejet s'obtient facilement par
l'observation de ces phénomènes brefs mais intenses.
\item Vents stellaires: les étoiles évoluées se caractérisent par une 
atmosphère extrêmement étendue et un dégagement énergétique
important. Sous cette forte pression radiative, la partie supérieure
de l'étoile peut être soufflée relâchant ainsi cette matière dans le
milieu interstellaire (figure~\ref{fig:M57}).
\end{itemize}

Les Supernovae ont longtemps été considérées comme la source
principale de rejet d'éléments lourds dans le milieu
interstellaire. Cette idée a été remise en cause par la faible
quantité de supernovae observées.  Plus particulièrement, on s'est
aperçu que la plupart des étoiles se débarrassent de 80\% de leur
masse avant leur mort, évitant ainsi de se retrouver avec une masse
finale supérieure à la masse critique de Chandrasekar (1.44
M$_\odot$), ce qui leur épargne une fin cataclysmique. Une inconnue
subsiste dans ce scénario: comment s'opère cette perte de masse?  Sous
l'effet de la pression de radiation, les grains peuvent permettre au
gaz d'acquérir une vitesse supérieure à la vitesse d'échappement ( 5 à
10 km/s). Pourtant, la condensation du gaz sous forme de poussières
nécessite une température bien inférieure à celle présente dans les
couches supérieures de l'atmosphère.  Il doit, par conséquent, exister
un premier mécanisme de propulsion, transportant la matière
suffisamment loin pour qu'il y ait condensation. Il semblerait que les
instabilités de l'étoile soient liées à ce phénomène. De larges
amplitudes de pulsation semblent en particulier être responsables
d'importantes pertes de matière \citep{1979ApJ...227..220W}. Les
instabilités régirait ainsi la suite de l'évolution stellaire.


\section{Les instabilités et modes d'oscillation}

On peut distinguer trois principaux types d'instabilités. Elles se
distinguent par des échelles de temps et de tailles différentes. Il
s'agit des instabilités thermique, dynamique et convective.

\subsection{Instabilité thermique}

La première source d'instabilité correspond à un emballement thermique.
Selon la loin des gaz parfaits:
\begin{equation}
P=\rho k T
\end{equation}
Ce qui peut aussi se traduire par:
\begin{equation}
\frac{d \, P}{P} = \frac{d \, \rho}{\rho} + \frac{d \, T}{T}
\end{equation}
Or, si l'on considère l'étoile à l'équilibre hydrostatique, on peut établir:
\begin{equation}
\frac{d\, P}{P} = 4/3 \frac{d \, \rho}{\rho}
\end{equation}
Soit
\begin{equation}
1/3 \frac{d \, \rho}{\rho} = \frac{d\, T}{T}
\end{equation}
Par conséquent, si le c\oe ur se contracte, $\rho$ augmente, ainsi que la
température. Cet accroissement de température permet de lutter contre
la contraction, permettant ainsi un retour à l'état d'origine. De
même, si le c\oe ur se dilate, la température diminue, permettant une
contraction du c\oe ur.

Cet équilibre est parfois rompu. C'est le cas lors du processus de
fusion au sein d'une couche. A une distance $r$ du centre de l'étoile et
à l'épaisseur $l$, l'équilibre hydrostatique
s'écrit:
\begin{equation}
\frac{d\,P}{P} = 4l/r \frac{d\,\rho}{\rho}
\end{equation}
Ainsi :
\begin{equation}
(4l/r - 1) \frac{d \, \rho}{\rho} = \frac{d \,  T}{T}
\end{equation}
Si $4l/r-1$ est négatif, l'expansion de la couche se traduit par une
augmentation de température et un emballement de la réaction de
fusion. Ceci se traduit concrètement par une pulsation de l'étoile
évoluée, expliquant des variations photométriques à des périodes de
plusieurs centaines d'années.

\subsection{Instabilité dynamique}
\label{sec:insta_dyn}

\begin{table}
\caption{Instabilités dynamiques}
\label{tb:periode_pulsations}
\centering
\begin{tabular}{lllll}
\hline
\hline
Type & Période & Population & Type spectral & Radial (R) ou \\
 & & & & non-radial (NR) \\
\hline
Miras & 100-700 jours & I, II & M, N, R, S & R  \\
RV Tauri & 20-150 jours & II & G, K & R \\
Cepheids & 1-50 jours & I & F6-K2 & R \\
RR Lyrae & 1.5-24 heures & II & A2-F2 & R \\
Le soleil & 5-10 min & I & G2 & NR \\
Naines blanches & 100-1000s & I, II & O, B2, A0 & NR \\
\hline
\end{tabular}
\begin{list}{}{}
\item Extrait de \citet{2001Theo_Astro}.
\end{list}
\end{table}

Elle correspond à un déplacement de matière à l'intérieur de
l'étoile. Supposons une contraction adiabatique d'une couche de
l'étoile.
\begin{equation}
	P_{\rm adia} V^\gamma=cst,
\end{equation}
La pression interne à cette couche va augmenter. Pour qu'il y ait
stabilité, il faut que la pression exercée sur cette couche augmente,
de manière à ramener le système à son état antérieur. La pression
due aux couches supérieures sous l'effet du champ
gravitationnel s'écrit: 
\begin{equation}
	P_{\rm grav}=\int_m^M Gm/(4 \pi r^4)  \, dm
\end{equation}
En considérant une dilatation infinitésimale de la couche ; $l=l+\varepsilon$:
\begin{equation}
	P_{\rm adia}'=P_{\rm adia}(1+3 \gamma \varepsilon)
\end{equation}
\begin{equation}
	P_{\rm grav}'=P_{\rm grav}(1+4 \varepsilon)
\end{equation}
Ainsi, pour qu'il y ait stabilité, il faut que $P_{\rm grav}' > P_{\rm
adia}'$ lorsque $\varepsilon > 0$. Soit:
\begin{equation}
	\gamma > 4/3
\end{equation}

Dans le cas d'un gaz monoatomique, $\gamma = 5/3$, ce qui confirme la
stabilité générale de l'étoile. Cependant, il existe des
exceptions. La plus notable est celle d'un gaz partiellement
ionisé. Lorsqu'il se contracte les électrons ont tendance à se
recombiner, et le gaz à perdre des particules. Pour un simple gaz
monoatomique ionisé entre 18 et 82\%, on peut démontrer
\citep{2001Stel_stru} que $\gamma < 4/3$.

Ce phénomène, observé à de multiples stades de l'évolution des
étoiles, est couramment appelé le ``$\kappa$ mécanisme''
\citep{1995ARA&A..33...75G,1996ARA&A..34..551G}. Une approche physique
en permet une meilleure compréhension.  Si l'on chauffe une couche de
gaz, elle se dilate, devient plus transparente, et peut ainsi émettre
son surplus d'énergie sous forme radiative.  Cependant, un gaz
partiellement ionisé, lorsqu'il se dilate, devient plus opaque du fait
de la recombinaison des électrons. Ceci augmente le réchauffement dû à
l'énergie irradiée par le centre de l'étoile, renforçant le phénomène
de dilatation. L'énergie nécessaire à l'existence de larges pulsations
peut ainsi être fournie. Néanmoins, ces couches de transitions entre
gaz ionisé et gaz non-ionisé sont localisées au sein de l'étoile. Il
existe principalement deux couches: celle correspondant à l'ionisation
de l'hydrogène ($1-1.5 \times 10^4$ K), et celle correspondant à
l'Hélium (He->He$^+$; $4 \times 10^4$ K). La position exacte de ces
couches dépend de la température effective de l'étoile. Une étoile
chaude ($T_{\rm eff} = 7500$ K) a ces couches très près de la surface,
ce qui l'empêche d'entraîner suffisamment de masse pour produire de
larges oscillations. {\it A contrario}, dans les étoiles ayant une
température de surface plus faible apparaissent d'importantes
oscillations. L'harmonique de résonance est alors sélectionnée en
fonction de la position de la couche d'ionisation. C'est, notamment,
ce qui permet aux Miras d'osciller sur le mode fondamental (cf
Table~\ref{tb:periode_pulsations}).


\subsection{Le phénomène de convection}
\label{sec:insta_conv}

Le phénomène de convection, bien que simple en son principe, s'avère
difficile à formaliser mathématiquement. Le concept peut être compris à partir d'un
déplacement vertical d'un petit élément de matière. Cet élément va
alors s'équilibrer en pression avec son nouvel environnement et se
dilater. Cette dilatation se traduit par une modification de sa
densité. Si elle devient plus faible que le milieu, la poussée
d'Archimède va l'entraîner encore plus vers le haut, produisant le
phénomène d'instabilité. Les paramètres moteurs de cette instabilité
sont le gradient de pression et le gradient de température. Un critère
d'existence de telles instabilités est celui de Schwarzschild:
\begin{equation}
	\frac{d\,\ln{T}}{d\,\ln{P}} > \frac{(\gamma -1)}{\gamma} \, .
\end{equation}
Dans l'atmosphère des étoiles, la convection apparaît dans les zones
faiblement ionisées, où l'opacité génère un important gradient de
température. Cette zone d'ionisation est très étendue dans
l'atmosphère relativement froide des étoiles évoluées. Le soleil,
quant à lui, présente aussi cette zone de convection, mais sur une
épaisseur beaucoup plus faible.

\subsection{le soleil}

\begin{figure}[h!] 
\centering 
\resizebox{\hsize}{!}{\includegraphics{Images/soleil1.eps}
\includegraphics{Images/soleil2.eps}}
   \caption{ Paramètres physiques du soleil \citep{1975ApJ...195..137S} }
   \label{fig:Schwar} 
\end{figure}


Bien que le soleil ne soit pas une étoile évoluée, notre grande
connaissance de son fonctionnement en fait une référence pour étudier
les instabilités. \citet{1975ApJ...195..137S} a accompli ce travail
dans le but de prédire les instabilités à la surface des
supergéantes. La figure~\ref{fig:Schwar} reproduit deux images de son
article qui représentent les différentes valeurs physiques à
l'intérieur de notre soleil. On observe les deux paramètres qui
caractérisent deux types d'instabilités
(paragraphes~\ref{sec:insta_dyn} et~\ref{sec:insta_conv}):
\begin{itemize}
\item Instabilité dynamique: l'opacité ($\kappa$)
\item Convection: le gradient de température $QTS = d\,\ln{T}/d\,\ln{P} - (\gamma-1)/\gamma$
\end{itemize}
Par un simple raisonnement géométrique, Schwarzchild associe ensuite
l'existence des granules à la zone convective, et les super-granules à
la zone d'ionisation de l'Hydrogène et de l'Hélium. Il en conclut que
ces types d'instabilités doivent exister dans les étoiles évoluées, mais à
un échelle beaucoup plus grande.

\section{Ma thèse dans ce contexte}


\begin{figure}[h]
\centering 
\includegraphics[width=9cm]{Images/Freyag.eps}
   \caption{ Simulation de l'effet de convection à la surface de super
   géantes \citep{2003csss...12.1024F} }
   \label{fig:Freytag} 
\end{figure}


Deux questions importantes justifient ce travail de thèse:
\begin{enumerate}
\item Quels sont les sources d'instabilité dans les étoiles évoluées? 
\item Comment la matière se trouve éjectée de l'atmosphère?
\end{enumerate}
Ces questions, intrinsèquement liées, ont de profondes répercussions
sur l'évolution stellaire et galactique. Cependant, parce que ces
phénomènes concernent la surface stellaire et son environnement
proche, la plupart des observations restent indirectes. Comme dans le
cas du soleil, nous nous attendons cependant à l'existence
d'instabilités dynamiques et convectives.

Concernant les phénomènes de convection, nous disposons, d'un coté,
des mesures de variations photométriques
\citep[récemment,][]{2006MNRAS.Kiss}, et de l'autre, des simulations 
d'atmosphères convectives (Figure~\ref{fig:Freytag}). Les instabilités
dyamiques se traduisent, elles, par des pulsations de grandes
amplitudes. Elle sont mieux connues car observées par interférométrie
\citep{2004A&A...426..279P} et disposent de sérieuses bases théoriques
\citep[par exemple][]{1996MNRAS.278...11F}.

Cependant, l'accélération initiale de la matière à la surface de
l'étoile est un mécanisme peu connu, notamment parce qu'il nécessite
la connaissance de l'instabilité de l'étoile. De nombreux modèles
existent cependant
\citep{1988ApJ...329..299B,1996A&A...307..481B,2006A&A...456.1001C},
mais sont confrontés à très peu d'observations. En l'absence de
résolution angulaire suffisante, les observations spectroscopiques ont
néanmoins permis d'apporter un certain nombre de contraintes à partir
des raies d'absorptions les plus énergétiques
\citep{1979ApJ...234..548H,1982ApJ...252..697H}.

L'objectif de ce travail de thèse est d'utiliser la haute résolutions
angulaire pour tenter de répondre à ces problématiques. Cependant,
face à la complexité des phénomènes, mesurer une fréquence spatiale
par interférométrie ne suffit plus. Il est nécessaire d'imager
entièrement la surface stellaire pour pouvoir dissocier les différents
mécanismes entrant en jeu.


==> image3.tex <==
\clearpage

\section{Les donnèes interférométriques}

\subsection{Principe général}

Un objet astrophysique se caractèrise par sa fonction continue de
distribution spatiale de brillance, allant de $-\infty$ à
$+\infty$. L'imagerie consiste à retrouver cette distribution. On peut
l'obtenir {\it via} un instrument imageur - télescope ou lunette - qui
permet de projeter une distribution d'intensité similaire sur un
détecteur. Néanmoins, lorsque l'on utilise un tel système, on modifie
cette fonction, en 1) la limitant en champ, 2) la limitant en
fréquence spatiale et 3) la convoluant par la réponse impulsionnelle
de l'instrument. L'image obtenue à travers un télescope est par
conséquent différente de la fonction de distribution de l'objet. Par
exemple, la théorie de la diffraction limite la résolution d'un
télescope à un facteur de la taille de celui-ci. Cette propriété est
une importante limitation technologique à l'obtention d'images à haute
résolution.

Pour s'en affranchir, on peut mesurer directement la valeur complexe
du champ électromagnétique provenant de l'objet observé. Le théorème
de Van Cittert-Zernike nous donne une relation directe entre la
distribution en flux d'un objet astrophysique $I(\alpha,\beta)$, et la
cohérence du champ à deux points distincts à la surface de la Terre:
\begin{equation}
  V(u,v)=TF(I(\alpha,\beta))
\end{equation}
où TF est la transformée Fourier normalisée, $(u,v)$ la base formée
par les deux points de mesures (en multiples de $\lambda$), et
$(\alpha,\beta)$ la coordonnée angulaire du flux observé (en radians).

Ainsi, la connaissance de la cohérence spatiale de la lumière nous
permet de reconstruire une image de l'objet, avec la transformée de
Fourier comme relation mathématique de passage.  En relevant la
cohérence du flux lumineux, on détermine une valeur correspondant à
une fréquence spatiale de l'objet. La résolution maximale de l'image
reconstruite sera limitée par la taille de la zone de mesure et la
qualité de reconstruction, par le nombre de mesures. Cependant, les
mesures ne peuvent couvrir de manière continue l'ensemble des
fréquences spatiales. Un algorithme de déconvolution devra être
utilisé pour déterminer celles manquantes. Un terme de régularisation
permettra de choisir la solution qui nous semble la plus appropriée
(voir paragraphe~\ref{sec:algo_rec_image}).

\subsection{IOTA (Infrared Optical Telescope Array)}

\begin{figure}[h!]
  \centering \includegraphics[width=15cm]{Images/Iota2.eps}
  \includegraphics[width=5cm]{Images/couverture_0.eps}
  \includegraphics[width=5cm]{Images/couverture_45.eps}
  \includegraphics[width=5cm]{Images/couverture_90.eps} \caption{ La
  figure du dessus représente le sommet de la montagne sur lequel est
  installé IOTA. Les télescopes sont situés sur des tripodes. Il
  existe 17 stations utilisables, mais toutes ne sont pas accessibles
  aux trois télescopes. Le télescope B, par exemple, est limité aux 5
  stations du bras Sud-Est. Le domaine du plan $u$-$v$ accessible est
  contraint par la géométrie de l'interféromètre, et par la position
  de l'étoile dans le ciel. Les fréquences spatiales sont représenté
  par les trois figures du dessous, ceci pour des étoiles observées
  pendant deux heures durant leur passage au méridien. La forme ``en
  sablier'' entraîne une résolution non uniforme que l'ont retrouvera
  lors de la reconstruction d'images. Note : parce qu'il est de
  tradition de représenter le ciel avec l'ouest à droite, les
  abscisses correspondent dans l'ensemble de cette thèse aux
  coordonnées $-u$ ($u$ correspond aux coordonnées Est et $v$ aux
  coodonnées Nord).  } \label{fig:IOTA}
\end{figure}


L'Infrared Optical Telescope Array (IOTA) est un interféromètre doté
de trois télescopes de 45 cm\citep{2003SPIE.4838...45T} fonctionnant
dans le proche infra-rouge. Ils sont situé sur le Mont Hopkins en
Arizona. IOTA est géré par un consortium américain rassemblant,
notamment, le {\em Smithsonian Astrophysical Observatory} et l'{\em
University of Massachusetts}. Les trois télescopes peuvent être
déplacé sur des rails, mais leur disposition reste déterminé par
l'emplacement de deux rails à 90 degrés l'un de l'autre. Le rail N-E
est d'une longueur de 35 mètres et dispose de stations tous les
multiples de 5 ou de 7 mètres. Le rail S-O dispose de 5 stations à 5,
7, 10, 14 et 15 mètres. L'ensemble des fréquences spatiales pouvant
être mesuré correspond aux combinaisons possibles projetées sur le
ciel. Cette projection dépend de la déclinaison de l'objet observé. La
longueur de base s'inscrit entre un minimum de 5 mètres et un maximum
de 38 mètres (figure~\ref{fig:IOTA}). Néanmoins, l'ensemble des
fréquences spatiales correspondant à une telle couverture n'est pas
forcément mesurable. De plus, le déplacement des télescopes nécessite
au mieux une demi-journée de travail, ce qui ne permet pas d'obtenir
plus de configurations que de nuits d'observations.

La recombinaison est de type co-axial, et est obtenue via un composant
en optique intégrée fabriqué au Laboratoire d'Astrophysique de
l'Observatoire de Grenoble. Le modulation, temporelle, est effectuée
par le déplacement de deux miroirs plans mus par des piezos.
La longueur d'onde de fonctionnement de l'optique intégrée correspond
à la bande H ($\lambda_0 = 1,65\,\mu$m et $\Delta \lambda =
0,35\,\mu$m). Certains tests fûrent neanmoins conduit par d'autres
équipes permettant d'obtenir des résultats en bande K ($\lambda_0 =
2,20\,\mu$m). L'ensemble de nos données ont été acquises en bande H.

\subsection{IONIC (Integrated Optics Near-infrared Interferometric
Camera)}

\begin{figure}
  \centering
  \includegraphics[width=6cm]{Images/composants-OI.eps} 
\vspace{.6cm}\\
  \includegraphics[width=12cm]{Images/IONIC.eps} \caption{ La photo
  est celle d'un composant en optique intégré fabriqué par le
  LAOG ({\it http://www-laog.obs.ujf-grenoble.fr/activites/hra/ionic/}).
  Elle donne une idée de la taille de ce type d'éléments de
  recombinaison. La figure du bas représente le schéma optique de
  IONIC utilisé sur IOTA.
  } \label{fig:schema_io}
\end{figure}


Afin de mesurer la cohérence spatiale des faisceaux provenant des
télescopes, la lumière est injectée dans des fibres optiques
monomodes. Ces fibres permettent un filtrage du rayonnemment de façon
à exclure les perturbations du front d'onde.  Les trois fibres sont
ensuite alignées sur un ``V-groove'' pour injecter la lumière dans un
recombinateur plan en optique intégrée \citep[IONIC
;][]{2003SPIE.4838.1099B}. Le circuit optique sépare ensuite le flux
provenant de chaques télescopes pour le recombiner par paires via
trois coupleurs intégrés (figure~\ref{fig:schema_io}). L'utilisation
de ce type de coupleur permet d'obtenir deux sorties interférométrique
par coupleur, chacune déphasé de $\pi$ par rapport à l'autre. Les
variations de l'intensité de couplage dans les fibres peuvent ainsi
être prisent en compte par l'intermédiaire de la matrice de tranfert
de l'optique intégrée. Celle-ci peut être obtenue par exemple en
injectant de la lumière séquentiellement dans les différentes voies.

\begin{figure}
  \centering
  \resizebox{\hsize}{!}{\includegraphics{Images/fringes-white.eps}}
  \caption{ Fenêtre de contrôle du suiveur de franges. On peut
  voir les franges correspondant aux trois bases, ainsi que leur
  spectre de puissance. On peut constater qu'une base est modulée à une
  fréquence double par rapport aux deux autres; ceci est dû à l'effet
  cumulé de la modulation des deux piezos. }
  \label{fig:Controle}
\end{figure}

Une correction rapide des variations photométriques consiste à
soustraire les deux voies déphasées issues de chaque coupleur. Ceci
peut être simplement explicité dans l'hypothése ou on néglige
l'influence des facteurs de transmissions des coupleurs.  Ainsi, pour
un rayonnement parfaitemet cohérent, les deux sorties
interférométriques fournissent :
\begin{eqnarray}
S_{12}(t)&=&I_1(t)+I_2(t)+ \sqrt{|I_1(t)| |I_2(t)|}  \cos(\omega t) \\
S_{12}^\star(t)&=&I_1(t)+I_2(t)+ \sqrt{|I_1(t)| |I_2(t)|}  \cos(\omega t +\pi) \,.
\end{eqnarray}
Si on applique la soustraction, on obtient :
\begin{eqnarray}
S_{12}(t)-S_{12}^\star(t)=2\sqrt{|I_1(t)| |I_2(t)|}  \cos(\omega t) \,.
\end{eqnarray}
Soit des oscillations à la moyenne indépendante des fluctuations
photométriques. Cependant, il s'agit du cas particulier où la
transmissions de chacun des coupleurs est de 50\% pour chacune des
voies. Un traitement plus fin, post observation, sera nécessaire pour
tenir compte de la matrice de transfert et des variations de
l'amplitude de modulation. Cette simple soustraction permet tout de
même une permière correction qui est utilisé par le
suiveur de frange. La figure~\ref{fig:Controle} est une copie de
l'écran du suiveur de frange. On peut voir les 3 figures
d'interférences, corrigées des variations photométriques.



\subsection{Traitement de données}
\label{sec:john_s}

\begin{figure}
  \centering \resizebox{\hsize}{!}{
  \includegraphics{Images/John_soft.eps}} \caption{ Apparence
  graphique du logiciel ``matrix2.script'' écrit par J. Monnier en
  langage IDL. Cette interface permet de selectionner les jeux de
  franges utile, et d'éliminer ceux qui semblent corrompus. En bas à
  droite figure la densité spectrale de puissance (en unités
  logarithmiques) d'ou seront extraites les visibilités non calibrés.}
  \label{fig:johhn_algo}
\end{figure}

Une série d'acquisition typique consiste en l'enregistrement d'une ou
deux série de 200 paquets de franges obtenus en environ 4
minutes. Chaque séquence est ensuite suivie de l'enregistrement du
fond et du flux obtenue avec chaque télescope indépendandament des
autres. Ceci permet la calibration par l'obtention de la matrice de
tranfert du recombinateur. Le temps total -- y compris le pointage --
d'une l'acquisition est d'ainsi environ 10-20 minutes.  Les
observations de la source sont interlacées par des séries
d'acquisitions identiques obtenues sur des calibrateurs. Ces
calibrateurs sont choisi pour être spatiallement proches de l'objet
d'intérêt scientifique ($\lessapprox 10$ degrés), de brillance
similaire, et surtout de visibilités connues (source ponctuelles où de
diamètres connus). Ces conditions permettent une mesure précise de la
fonction de transfert de l'interférométre.

La réduction des données interférométrique s'est faite sous IDL par un
logiciel écrit par John Monnier de l'{\em University of Michigan}
\citep[voir par exemple ;][]{2004ApJ...602L..57M}. Ce logiciel se
compose principalement de deux parties. La première permet de calculer
les densités spectrales de puissance, et la seconde de calibrer les
visibilités au carré. La figure~\ref{fig:johhn_algo} est une copie de
l'écran correspondant à la sélection des franges. Sur cette figure est
sélection un set de 200 acquisitions, que l'on peut ainsi sélectionner
ou éliminer en fonction de leur qualité. Ceci permet ainsi d'éliminer
des données qui peuvent êtres corrompues par un seeing trop important,
ou alors un problème instrumental comme l'oscillation de la ligne à
retard. A partir du pic frange que l'on peut observer dans la densité
spectrale de puissance, le logiciel fournit une visibilité au carré
$V^2$, qui sera ensuite normalisé par la visibilité des calibrateurs.

\subsection{Clôtures de phase}

\begin{figure}[h]
  \centering \includegraphics[width=11cm]{Images/Clotur_schema.eps}
  \caption{ Schéma d'un interférométre à trois télescopes illustrant
  l'utilité de la mesure de clôture de phase. Chaque télescope recoit
  le rayonnement astrophysique déphasé de l'effet d'un piston
  atmosphérique, introduit par les variations d'indices des couches
  turbulentes de l'atmosphère. La clôture de phase permets de
  s'affranchir de ces termes $\phi_1$, $\phi_2$ et $\phi_3$.  }
  \label{fig:schema_clo}
\end{figure}

Parralellement à l'extraction des visibilités au carré, le logiciel de
J. Monnier mesure aussi une information sur la phase des
visibilités. Il s'agit des clôtures de phase (CP).

La method de clôture de phase fut développé initialement par les
radiointerférométristes \citep{1958MNRAS.118..276J} pour s'affranchir
d'un terme de déphasage sur des données obtenues par interférométrie
hétérodyne. L'idée peut être comprise par un le biais de la
figure~\ref{fig:schema_clo}. Dans ce schema, le rayonnement issue de
la source astrophysique est déphasé d'un terme $\phi_i$ lorsqu'il
arrive sur chacun des télescopes. Ce terme peut être du à un piston
atmosphérique ou à un probléme de calibration astrométrique. Le phase
mesuré entre les telescopes 1-2, 1-3 et 2-3 est la somme de la phase
de l'objet astrophysique (respectivement $\Phi_{12}$, $\Phi_{12}$ et
$\Phi_{12}$) et de différence la différence des pistons
atmosphériques. Nos mesurons de cette maière une phase
$\Phi^\ddagger_{ij}$ tel que:
\begin{equation}
\Phi^\ddagger_{ij}=\Phi_{ij}+\phi_j-\phi_i \,.
\label{eq:cloture_s}
\end{equation}
La clôture de phase est la somme des trois phases obtenues par ces
trois télescopes :
\begin{equation}
\Phi^{CP}_{ijk}=\Phi^\ddagger_{ij}+\Phi^\ddagger_{jk}+\Phi^\ddagger_{ki}\,.
\end{equation}
Ainsi, en appliquant l'équation~\ref{eq:cloture_s}, on peut montrer que
$\Phi^{CP}_{ijk}$ est indépendant des termes de piston atmospheriques,
et qu'il vaut :
\begin{equation}
\Phi^{CP}_{ijk}=\Phi_{ij}+\Phi_{jk}+\Phi_{ki}\,.
\end{equation}

En pratique, les clôtures de phases sont obtenues par l'intermédiaire
du bispectre. Nous aurons l'occasion de revoir ce point
section~\ref{sec:clot}. Le concept mathématique, dont notament
l'influence du bruit de photon, est étudié plus en détail dans la
thèse de \citet{Thiebaut1994:PhD}.


Les clôtures de phases permettent ainsi d'obtenir une information
partielle sur la phase de l'objet astrophysique. L'avantage de cet
estimateur est sa grande robustesse aux perturbations
astrophysiques. Nous verrons que nos données de clôtures de phases
sont souvent obtenues avec des précisions de quelques degrès. Ces
clôtures de phases ont deux propriétés fondamentale importantes
\begin{itemize}
\item Elles sont invariantes par rapport à la position de l'objet dans
le ciel. Ainsi, il n'est pas possible de faire de l'astrométrie
absolue, mais uniquement relative. Nous verrons par la suite que les
reconstructions ne sont pas forcement centrées par rapport à la
position {\it zero}. Ceci résulte tout simplement de l'abscence de
contrainte sur la position. En pratique, nous utiliseront un terme
régulateur visant à centrer l'image (section~\ref{sec:algo_rec_image})
\item Elles sont nulle dans le cas d'un objet centro-symmétrique. Plus
exactement, elles sont sois nulles, soit égale à $\pi$ lorsque la
visibilité est négative. Ceci permet deux
choses. D'abord de révéler clairement la présence de lobes où la
visibilité s'inverse. Ensuite, de révéler nettement lorsque l'objet
observé est assymétrique. Nous verrons que ces deux propiétés
permettent une première interprétations rapides de données
interférométriques.
\end{itemize}

\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Les observations}

\begin{table}[h]
\caption{Missions d'observations}
\label{tb:missions}
\centering
\begin{tabular}{llr}
\hline
\hline
Période & Objet & Observateurs \\
\hline
19 -- 28 Octobre 2004 &  -- {\it Mauvais temps} -- & GP, SL, SM et JW\\
 21 -- 31 Mai 2005 & $\chi$ Cyg, CH Cyg & SL et SM\\
 4 -- 16 Octobre 2005 & $\chi$ Cyg, Mira, Bételgeuse & GP, SL et XH\\
 28 Mars -- 6 Avril 2006 & $\chi$ Cyg, R leo & SL, XH et PS \\
 10 -- 15 Mai 2006 & $\chi$ Cyg, R leo, Arcturus, $\mu$ Cep & SL, AP
 et PS \\
\hline
\end{tabular}
\begin{list}{}
{\vspace{.2cm}}
\item[-] Marc Lacasse étant le technicien responsable de l'interférométre,
 il était généralement présent lors des missions d'observations. De
 plus, était présent : GP; Guy Perrin, SL; Sylvestre Lacour, SM; Serge
 Meimon, JW; Julien Woilez, XH; Xavier Haubois, PS; Peter Schuller et
 AP; Anne Poncelet.
\end{list}
\end{table}

\subsection{L'objectif}

L'objectif premier de ces missions d'observation est de parvenir à
imager par interférométrie la surface stellaire des étoiles évoluées.
L'obtention de l'information de phase -- via les clôtures de phase --
est nécessaire pour la reconstruction d'une image complexe. Cette
information est devenue accessible sur un interférométre fibré lors de
l'ouverture à la communauté astrophysique de l'observatoire
IOTA. Malgrès cela, la pluspart des publications actuelles portent
uniquement sur une analyse paramétrique des données. Concernant IOTA,
nous ponvons par exemple siter les résultats de
\citet{2006ApJ...647..444M} sur les étoiles Herbig Ae/Be, où les
auteurs ajustent des modéles de disques d'accrétion sur les clôtures
de phase. Nous pouvons aussi prendre pour exemple les travaux récents
de \citet{2006astro.ph..7156R} qui ont mesuré des clôtures de phases
sur 56 étoiles de la branche asymtoptique des géantes. Dans le cas de
leur analyse paramètrique des donées, seule quelques mesures par
étoiles suffirent.

Notre approche est plus difficile car l'imagerie nécessite une
connaisance exaustive du plan des fréquences spatiales. Ceci rend nos
travaux novateurs au respect du travail de
\citet{2006astro.ph..7156R}. Alors qu'ils se sont plutôt
focalisé sur l'observation d'une grande quantité d'objets, nous avons
choisi de limiter le nombres d'étoiles observées pour étendre autant
que possible la couverture du plan $u$-$v$. Cette approche à
l'inconvéniant de nécessiter des changement fréquent de la
configuration de l'interférométre, avec tout les problèmes technique
que le déplacement des télescopes imposent.

\subsection{Les missions d'observations}


\begin{table}
\caption{Liste des étoiles évoluées étudiées}
\label{tb:star}
\centering
\begin{tabular}{lrrccc}
\hline
\hline
 Objet & \multicolumn{1}{c}{$\alpha$} & \multicolumn{1}{c}{$\delta$} & Type spectral & Type & Période(s)  \\
\hline
Arcturus & 14 15 39.67 & +19 10 56.7 & K1.5III & Géante &\\
CH Cyg & 19 24 33.07 & +50 14 29.1 & M7IIIv & Symbiotique & 100-155$^{\mathrm{a}}$\\
$\chi$ Cyg & 19 50 33.92 & +32 54 50.6 & MS & Mira & 408 \\
R leo & 09 47 33.49 & +11 25 43.6 & M8IIIe & Mira & 312 \\
Mira & 02 19 20.79 & -02 58 39.5 & M2-M7 IIIe & Mira & 332 \\
Bételgeuse & 05 55 10.31 & +07 24 25.4 & M2Iab & Supergéante& 388, 2050$^{\mathrm{b}}$\\
$\mu$ Cep & 21 43 30.46 & +58 46 48.2 & M2Ia & Supergéante & 860, 4400$^{\mathrm{b}}$\\
\hline
\end{tabular}
\begin{list}{}{}
\item[$^{\mathrm{a}}$] \citet{1992JAVSO..21...23K}
\item[$^{\mathrm{b}}$] \citet{2006MNRAS.Kiss}
\end{list}
\end{table}

Ceci contraint à des missions d'observations plutôt longues, avec des
durées vairables entre 20 et 10 jours. Il y a eu 5 missions
d'observations au Mont Hopkins qui se sont déroulées d'Octobre 2004 à
Mai 2006 (tableau~\ref{tb:missions}). \`A noter la première et la
dernière mission. La première s'est traduite par quinze jours de
mauvais temps, et la dernière par l'utilisation d'un tout nouveau mode
de fonctionnement, qui a permis de disperser les franges et d'obtenir
une information spectro-interférométrique. Le tableau~\ref{tb:star}
répertorie les objets observés au cours de ces diférentes
missions. Toutes sont des étoiles évoluées de type Mira, Géante ou
Supergéante rouge.

\subsection{Les données}



\begin{table}
\caption{Configurations des télescopes}
\label{tb:Config}
\centering
\begin{tabular}{lccccc}
\hline
\hline
Date & Configuration & \multicolumn{4}{c}{Objet} \\
\hline
24 Mai 2005&	A35-B15-C0&	&CH Cyg	\\
25 Mai 2005&	A15-B15-C0&	$\chi$ Cyg	\\
27 Mai 2005&	A15-B15-C5&	$\chi$ Cyg	\\
31 Mai 2005&	A25-B15-C10&	$\chi$ Cyg&CH Cyg	\\
1 Juin 2005&	A35-B15-C10&	$\chi$ Cyg	\\
\hline
5 Octobre 2005&	A5-B5-C0&	$\chi$ Cyg&	\\
6 Octobre 2005&	''&	$\chi$ Cyg&	Mira	\\
7 Octobre 2005&	''&	$\chi$ Cyg&	Mira&	Bételgeuse	\\
8 Octobre 2005&	A5-B15-C0&	$\chi$ Cyg&	Mira&	Bételgeuse	\\
9 Octobre 2005&	''&	$\chi$ Cyg&	\\
10 Octobre 2005&	A15-B15-C0&	$\chi$ Cyg&&	Bételgeuse	\\
11 Octobre 2005&	''&	$\chi$ Cyg&	Mira&	Bételgeuse	\\
12 Octobre 2005&	A25-B15-C0&	$\chi$ Cyg&	Mira&	Bételgeuse	\\
13 Octobre 2005&	''&	$\chi$ Cyg&	Mira	\\
15 Octobre 2005&	A30-B15-C15&&	Mira	\\
16 Octobre 2005&	''&&&	Bételgeuse	\\
\hline
29 Mars 2006&	A15-B15-C0&	$\chi$ Cyg&	R leo 	\\
31 Mars 2006&   "&	$\chi$ Cyg	\\
2 Avril 2006&	A5-B5-C0&	$\chi$ Cyg&	R leo	\\
3 Avril 2006&	A5-B10-C0&&	R leo	\\
4 Avril 2006&	A25-B10-C0&&	R leo	\\
7 Avril 2006&	A30-B15-C0&	$\chi$ Cyg&	R leo	\\
\hline
11 Mai 2006&	A15-B5-C10&	$\chi$ Cyg&	R leo& Arcturus&	$\mu$ Cep	\\
12 Mai 2006&	A15-B5-C0&	$\chi$ Cyg&	R leo& Arcturus&	$\mu$ Cep	\\
13 Mai 2006&	A15-B15-C0&	$\chi$ Cyg&	R leo& Arcturus	\\
14 Mai 2006&	A30-B15-C0&	$\chi$ Cyg&	R leo& Arcturus&	$\mu$ Cep	\\
15 Mai 2006&	A35-B15-C21&	$\chi$ Cyg&	R leo& &$\mu$ Cep	\\
16 Mai 2006&	A35-B15-C25&	$\chi$ Cyg&	R leo& Arcturus&	$\mu$ Cep		\\
\hline
\end{tabular}
\begin{list}{}{}
\item Les configurations utilisent comme notations les locations des
télescopes A, B et C, qui correspondent respectivement aux rails NE,
SE et NE.
\end{list}
\end{table}


\begin{table}[h]
\caption{Liste des calibrateurs utilisés}
\label{tb:calib_t}
\centering
\begin{tabular}{lcrr}
\hline
\hline
Calibrateur & Type Spectral  & Diamètre & Objet \\
\hline
\hline
HD\,176670 &    K2.5\,III   & 2,330 $\pm$  0,026 & $\chi$ cyg\\
HD\,177808   &    M0\,III      & 2,32  $\pm$  0,030 & $\chi$ cyg\\
HD\,180450 &    M0\,III     & 2,770  $\pm$ 0,032 & $\chi$ cyg\\
HD\,186619 &    M0\,IIIab   & 2,190  $\pm$ 0,025 & $\chi$ cyg\\
HD\,188149 &    K4\,III     & 1,490  $\pm$ 0,020 & $\chi$ cyg\\
HD\,197989 &    K0\,III     & 4,440  $\pm$ 0,048 & $\chi$ cyg\\
HD\,8512 &  K0\,IIIb  &    2,69 $\pm$   0,030 & Mira \\
HD\,16212 & M0\,III  &   3,02 $\pm$   0,032 & Mira\\
HD\,36167  & K5\,III  &     3,56 $\pm$  0,057 & Bételgeuse \\
HD\,48433  & K0.5\,III  &     2,07 $\pm$  0,027 & Bételgeuse \\
HD\,82381 & K2.5\,IIIb  & 2,09  $\pm$ 0,026 & R leo \\
HD\,87837 & K3.5\,IIIb  &  3,22 $\pm$  0,049 & R leo \\
HD\,120477  & K5.5\,III  &   4,46 $\pm$  0,050 & Arcturus\\
HD\,125560  & K3\,III  &   1,91 $\pm$  0,021 & Arcturus\\
HD\,129972   & G8.5III  &  1,54  $\pm$ 0,020 & Arcturus\\
HD\,176670 &    K2.5\,III   & 2,330 $\pm$  0,026 & $\chi$ cyg\\
HD\,177808   &    M0 III      & 2,32  $\pm$  0,030 & $\chi$ cyg\\
HD\,180450 &    M0\,III     & 2,770  $\pm$ 0,032 & $\chi$ cyg\\
HD\,186619 &    M0\,IIIab   & 2,190  $\pm$ 0,025 & $\chi$ cyg\\
HD\,188149 &    K4\,III     & 1,490  $\pm$ 0,020 & $\chi$ cyg\\
HD\,197989 &    K0\,III     & 4,440  $\pm$ 0,048 & $\chi$ cyg\\
HD\,198149  &  K0\,IV &  2,68 $\pm$  0,0290 & $\mu$ Cep \\
\hline
\end{tabular}
\begin{list}{}{}
\item Les calibrateurs sont issus des
catalogues de \citet{2002A&A...393..183B} et de \citet{2006A&A...447..783M}
\end{list}
\end{table}

Les données ont été réduite par le logiciel présenté
section~\ref{sec:john_s}. Les données sont acquisent lorsque deux
voies au moins peuvent detecter les franges. Cette condition permet
d'en déduire leur présence dans la troisiéme fenétre d'intégration,
même si elle ne sont pas instantanément détectables. De cette manière
(une technique appellé ``boot-strapping'' en anglais) nous avons ainsi
pu mesurer des CP et V$^2$ même pour des amplitudes de franges noyées
dans le bruit de photon. Figure~\ref{fig:Donnees_6} par exemple présente des
mesures de V$^2$ inférieures à $10^{-4}$. La liste des configurations
utilisé est présenté tableu~\ref{tb:Config}.

Les étoiles de calibration utilisées sont listées
tableau~\ref{tb:calib_t}. Celles ci ont était choisi a partir des
catalogues de \citet{2002A&A...393..183B} et de
\citet{2006A&A...447..783M}, sur des critéres de proximité spatiale et
de magnitude. Sur l'ensemble des calibrateurs, nous avons constaté des
erreurs sur les Visibilités au carrés de l'ordre de 2\%. Ces erreurs
peuvent être du à des incertitudes dans le calcul de leur diamètres,
ou à des variations de la fonction de transfer instrumental
inférieures sur des périodes inférieurs à 30 minutes. Pour tenir
compte de ces incertitudes, nous avons rajouté quadratiquement une
erreur sur les visibilités normalisé de 2\%.

Les clôtures de phases se sont révélées extraimement fiables, avec des
variations entre les différents calibrateurs au cours de la nuit de
l'ordre du degrés. Ceci est du à la qualité et à la miniaturisation du
composant d'optique intégré, ainsi très faiblement affecté par
d'éventuelles variations de température (Le laboratoire d'optique
d'étant pas une salle isolé, nous y avons constaté des changements de
température de plusieurs degrés). Une autre source d'erreurs sur les
clôture réside dans le différence entre le type spectral des
calibrateurs (G8 à M0) et des étoiles évoluées que nous avons
étudiés. En pratique, des test ont été éffectué et révélent des
vairations trés faibles ($\approx 0,5°$) entre des étoiles chaude (B8)
et froide (M3) \citep{Rag_CP_Cloture}. 

Figures~\ref{fig:Donnees_1},~\ref{fig:Donnees_2},~\ref{fig:Donnees_3},~\ref{fig:Donnees_4},~\ref{fig:Donnees_5}
et~\ref{fig:Donnees_6} représentes les visibilités au carré et les
clotures de phases calibrés.  L'ordonné des visibilités est en
logarithme, de façon à mettre en valeur l'information apporté par les
faibles visibilités. Les clôtures de phases sont comprises entre -180
et 180 degrés. Figure~\ref{fig:Donnees_1} correspond à la mission de
Mai 2005, figures~\ref{fig:Donnees_2} et~\ref{fig:Donnees_3} à la
mission d'Octobre 2005, figure~\ref{fig:Donnees_4} à la mission de
Mars 2006 et figures~\ref{fig:Donnees_5} et~\ref{fig:Donnees_6} à la
mission de Mai 2006. Une première analyse de ces données est effectué
dans les légende, de façon à indiquer les points notables de chacunes
des observations.

A la vue de ces données, on peut remarquer premiérement une
progression en terme de qualité et d'efficacité. Ceci est du bien sûr à
l'expérience de l'équipe d'observation, mais aussi aux développement
effectués par l'équipe technique responsable de l'interférométre. On
peut par exemple comparer la premiere mission d'observation (11 nuits)
à la derniére (6 nuits). Lors de la première mission, nous n'avons pu
observer qu'avec un maximum de 4 configurations sur deux objets. Lors
de la dernière mission, nous déplacions les télescopes chaques
journées et observions trois à quatres objets. Ceci a tenu aussi en
parti à des conditions météologiques favorables. Ces conditions nous
ont permit nottament d'obtenir des données avec de grandes précisions,
comme nous pouvons le voir sur Arcturus (nous pouvons voir des mesures
de visibilités au carrées inférieures à $10^{-4}$
figure~\ref{fig:Donnees_5}). A la lumières des données obtenus lors de
cette derniére mission d'observation, la fermeture récene de l'interférométre
IOTA est d'autant plus regrétable.


\begin{figure}
\centering
\resizebox{\hsize}{!}{
\includegraphics{Images/ChiCyg_Mai2005V2_data.eps}
\includegraphics{Images/ChiCyg_Mai2005CP_data.eps}
}
{\vspace{.3cm}}
\resizebox{\hsize}{!}{
\includegraphics{Images/CH_CygV2_data.eps}
\includegraphics{Images/CH_CygCP_data.eps}
} \caption{ V$^2$ et CP obtenues au cours de la premiére mission
   d'observation. A configurations différentes ont été utilisé sur
   $\chi$ Cyg, et 2 sur CH Cyg. Nous pouvons distinguer clairement le
   zero du premier lobe de $\chi$ Cyg, ce qui n'est pas le cas pour CH
   Cyg, ayant un diamètre angulaire plus grand. Les clôtures de phase
   indiquent de forte assymétrie sur la brillance de la surface
   stellaire de $\chi$ Cyg.}
   \label{fig:Donnees_1}
\end{figure}

\begin{figure}
\centering
\resizebox{\hsize}{!}{
\includegraphics{Images/ChiCyg_Octobre2005V2_data.eps}
\includegraphics{Images/ChiCyg_Octobre2005CP_data.eps}
}
{\vspace{.3cm}}
\resizebox{\hsize}{!}{
\includegraphics{Images/MiraV2_data.eps}
\includegraphics{Images/MiraCP_data.eps}
} \caption{ V$^2$ et CP obtenues au cours de la seconde mission
   d'observation. $\chi$ Cyg, toujours assymétrique, présente un zéro
   à une fréquence spatiale plus petite, caractéristique d'un diamètre
   plus grand. Les données de Mira témoingnent d'une a ssymétrie
   encore plus grande, qui peut être vu à la fois sur les clôture de
   phases et sur les visibilités. En effet, la dispersion observé aux
   fréquences proches de 8 M$\lambda$ ne sont pas du à un bruit, mais
   bien à une dépence des visibilité par rapport à l'angle de
   projection des différentes bases.}  \label{fig:Donnees_2}
\end{figure}

\begin{figure}
\centering
\resizebox{\hsize}{!}{
\includegraphics{Images/BetelV2_data.eps} 
\includegraphics{Images/BetelCP_data.eps}
} \caption{ Observation de Betelgeuse au cours de la mission
   d'observation d'Octobre 2005. On peut observé quatre lobes sur
   visibilités. Le premier zéro ce situe pour une fréquence spatiame
   d'environ 5 M$\lambda$, le second à 10 M$\lambda$, et le troisième
   autour de 15 M$\lambda$. Ceci est possible grace au large diamètre
   angulaire de Betelgeuse, qui est de 43,3 mas.  Les clôtures de
   phases indiquent des assymétries même si plus faibles que celles
   observées sur $\chi$ Cyg. Par exemple, la base A5-B15-C0
   correspondant au second lobe indique des clôtures de quelques
   degrés, à la différence de $\chi$ Cyg (figure~\ref{fig:Donnees_1})
   qui indique des valeurs de l'ordre de 120 degrés. L'absence de
   déphasage de 180 sur les CP est fortruit et est uniquement dû au
   hasard du choix des configurations.}  \label{fig:Donnees_3}
\end{figure}

\begin{figure}
\centering
\resizebox{\hsize}{!}{
\includegraphics{Images/ChiCyg_Mars2006V2_data.eps}
\includegraphics{Images/ChiCyg_Mars2006CP_data.eps}
}
{\vspace{.3cm}}
\resizebox{\hsize}{!}{
\includegraphics{Images/R_leo_Mars2006V2_data.eps}
\includegraphics{Images/R_leo_Mars2006CP_data.eps}
} \caption{ V$^2$ et CP obtenues au cours de la troisième mission
   d'observation. Les données de $\chi$ Cyg sont trés spartiates dù au
   passage au méridiens tardif de l'étoile, et donc à la complexité de
   ces observations. Le point de visibilité très faible à 15
   M$\lambda$ pourrait indiquer une petite taille angulaire (comparés
   aux données de Mai 2005). Nous verrons cependant
   (figure~\ref{fig:Data_Mar06}) que cette valeur est due à
   l'assymérie.  Les données sur R leo sont de très bonne qualité,
   avec une assymétrie importante pouvant être vu à la fois sur les
   visibilités et sur les clôures de phases. } \label{fig:Donnees_4}
\end{figure}

\begin{figure}
\centering
\resizebox{\hsize}{!}{
\includegraphics{Images/ChiCyg_Mai2006V2_data.eps}
\includegraphics{Images/ChiCyg_Mai2006CP_data.eps}
}
{\vspace{.3cm}}
\resizebox{\hsize}{!}{
\includegraphics{Images/R_leoV2_data.eps}
\includegraphics{Images/R_leoCP_data.eps}
} \caption{ V$^2$ et CP obtenues au cours de la dernière mission
   d'observation. Lors de cette mission, nous avons utilisé un prisme
   positioné entre le détecteur et le recombinateur IONIC. Ceci nous à
   permis de disperser les franges sur septs canaux, permettant ainsi
   des mesures interférométiques simulatnément à sept longueurs
   d'ondes différentes. Chaques longueurs d'ondes sont ici représenté
   par une couleur. Ont peut noté un passage à zéro des visibilité de
   $\chi$ Cyg ``confu'', et le faible troisiéme lobe de R
   leo. L'information spectrale sur les clôtures de phase est elle
   aussi très intéressante, car leur attitude permet de contrainte
   spectralement l'asymétrie (voir section~\ref{sec:dispertion})}
   \label{fig:Donnees_5}
\end{figure}

\begin{figure}
\centering
\resizebox{\hsize}{!}{
\includegraphics{Images/ArcturusV2_data.eps}
\includegraphics{Images/ArcturusCP_data.eps}
}
{\vspace{.3cm}}
\resizebox{\hsize}{!}{
\includegraphics{Images/Mu_CepV2_data.eps}
\includegraphics{Images/Mu_CepCP_data.eps}
} \caption{ V$^2$ et CP obtenues au cours de la dernière mission
   d'observation. Les données Arcturus (V$^2$ et CP) sont parmis les
   plus belles de notre jeu. Ces mesures montrent ainsi clairement la
   qualité de mesure que peut fournir un interférométre fibré. Les
   clôtures de phases passent nettement de 0 à 180 degrés lorsque le
   zéro est franchi, et des visibilités très faibles ont put être
   mesuré grace à la technique de ``boot-strapping''. Les données sur
   $\mu$ Cep sont aussi intéressante. Une asymétrie peut être détecté
   à la fois sur les visibilités. Cette asymétrie se retrouve
   clairement sur les clôture de phases, qui passent progressivement
   de 5 à 165 degrés. Ce passage étant dû à la base A35-B15, nous le
   retrouvons au cours de trois nuits différentes, prouvant bien la
   répétabilité de ces observations. } \label{fig:Donnees_6}
\end{figure}

\clearpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{L'algorithme de reconstruction d'image}
\label{sec:algo_rec_image}

\subsection{L'attache aux données}

\subsection{Modèle \textit{a priori}}


Le principe de la reconstruction en aveugle consiste à combler un
manque d'information - dans notre cas, les fréquences spatiales
inconnues - par un terme régulateur. On parle d'approche
Bayésienne. Lors d'un ajustement classique, on cherche les valeurs des
paramètres qui minimisent le maximum de vraisemblance ($\chi^2$). Dans
notre cas, on cherche l'image $I(\alpha,\beta)$ qui minimise
la fonction:
\begin{equation}
\chi^2 + \lambda f(I(\alpha,\beta)) \, , 
\end{equation}
$\lambda$ étant un hyperparamètre permettant de régler le poids de la
 fonction de régularisation ($f$) par rapport au $\chi^2$.

L'algorithme de reconstruction a été développé à l'observatoire de
Lyon, sous la direction d'\`Eric Thiebaut. Celui-ci utilise la fonction
de régularisation:
\begin{equation}
f(I(\alpha,\beta))=\frac{1}{1+(\alpha^2+\beta^2)/w^2}
\end{equation}
avec $w$ un paramètre à choisir en fonction de la nature de l'objet
observé. Cette fonction de régularisation joue le rôle d'un
``ressort'', c'est-à-dire que si la contrainte des données devient
faible, l'image aura tendance à se rapprocher d'une Lorentzienne.
Dans le cas de la métaphore du ressort, l'hyperparamètre correspond à
la constante de raideur, et devra donc étre réglé par l'utilisateur
avec soin. La Figure~\ref{fig:hyper} montre l'influence de ce
paramètre sur la reconstruction d'image. Si le paramètre est trop
grand, l'image est fortement contrainte par la fonction de
régularisation. Si le paramètre est trop faible, cela laisse
l'algorithme libre de faire de la sur-résolution ce qui peut faire
apparaître des artefacts. L'hyperparamètre a donc été choisi pour une
valeur intermédiaire, soit $3\times 10^7$.

\begin{figure}[h]
\centering
\resizebox{\hsize}{!}{
\includegraphics{Images/V1_1e6.eps}
\includegraphics{Images/V1_1e8.eps}
\includegraphics{Images/V1_1e12.eps}
}
   \caption{ Reconstruction d'une source ponctuelle simulée à
   partir de la couverture fréquentielle d'Arcturus et d'un objet
   ponctuel. Nous pouvons voir l'effet de l'hyperparamètre de valeur:
   $10^6$, $10^8$ et $10^{12}$ (de gauche à droite). Sur l'image de
   droite, on retrouve la Lorentzienne qui correspond à la fonction de
   rappel; l'hyperparamètre a donc une valeur trop élevée. A l'opposé,
   l'image de gauche montre une résolution supérieure à celle de
   l'interféromètre (qui est de 9 $\times$ 22 mas); l'hyperparamètre
   est donc trop faible. Enfin, sur l'image centrale, on obtient une
   image proche de celle correspondant à un telescope de la taille
   d'IOTA; l'hyperparamètre est donc bon. Ce choix n'est cependant pas
   forcément le même quel que soit l'objet, car il dépend aussi de la
   couverture fréquentielle et de la qualité des données.  }
   \label{fig:hyper}
\end{figure}

\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Imagerie en aveugle}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Arcturus}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \begin{figure}[h]
   \centering
   \includegraphics[width=6.2cm]{Images/UV_plane_Aboo.eps}
   \includegraphics[width=7cm]{Images/Image_Eric_Aboo.eps}
      \caption{ Partie gauche: Plan $u$-$v$ couvert par une séquence
      d'observation de 5 jours. La couverture des fréquences spatiales
      est plutôt homogène, malgré une direction (N-NE) privilègiée.
      L'utilisation du mode dispersé permet de bénéficier de
      l'influence de la longueur d'onde sur la fréquence spatiale
      mesurée. La condition étant de ne pas avoir un objet trop
      chromatique. Partie droite: Image reconstruite par le logiciel
      Mira d'\`Eric Thiébaut. Sur cette image, on résout clairement
      la géante rouge, sans y voir la présence d'un compagnon ou d'une
      asymétrie flagrante. }
         \label{fig:Arcturus}
   \end{figure}

Les géantes de type K sont souvent utilisées comme sources de
références pour l'étude des étoiles évoluées. Elles sont un bon
compromis entre luminosité et complexité. En effet, leur atmosphère
très compacte (du moins par rapport à l'ensemble des autres étoiles
évoluées) induit de faibles pulsations et un phénomène de convection
limité. En conséquence, on s'attend à une atmosphère simple sans
présence de couches moléculaires à grande distance de la
photospère. Arcturus (K1.5-2III, alpha Bootis) est l'une de ces
étoiles les plus connues. Elle a déjà été observée dans le visible par
l'interféromètre Mark III \citep{1996A&A...312..160Q}, ce qui a
confirmé les modèles existants, notamment la présence d'un
assombrissement centre-bord important \citep{1977A&A....61..809M}. Des
observations plus récentes en infrarouge proche
\citep{2005A&A...435..289V} suggèrent cependant l'existence d'un
compagnon à cette étoile. Si cela était confirmé, un tel résultat
aurait des conséquences importantes, cet objet étant considéré comme
une référence photométrique et spectrale
\citep[notamment pour ISO; ][]{2003A&A...400..709D}.

Les données correspondent à 5 nuits d'observation du 10 au 15 Mai
2006. Lors de ces nuits, nous avons pu utiliser le mode dispersé
d'IOTA. L'image obtenue (figure~\ref{fig:Arcturus}) correspond à un
disque circulaire doté d'un assombrissement semblant plus prononcé sur
l'axe horizontal. Ceci est dû à une résolution plus faible dans ce
sens, les bases disponibles de l'interféromètre IOTA limitant la
résolution selon l'axe Est-Ouest. Aucun compagnon n'a pu être mis en
évidence.


   \begin{figure}
   \centering
   \includegraphics[width=5.4cm]{Images/UV_plane_Chi_Cyg_Mai05.eps}
   \includegraphics[width=6.1cm]{Images/Image_Eric_Chi_Cyg_Mai05.eps}
   \includegraphics[width=5.4cm]{Images/UV_plane_Chi_Cyg_Oct05.eps}
   \includegraphics[width=6.1cm]{Images/Image_Eric_Chi_Cyg_Oct05.eps}
   \includegraphics[width=5.4cm]{Images/UV_plane_Chi_Cyg_Mar06.eps}
   \includegraphics[width=6.1cm]{Images/Image_Eric_Chi_Cyg_Mar06.eps}
   \includegraphics[width=5.4cm]{Images/UV_plane_Chi_Cyg_Mai06.eps}
   \includegraphics[width=6.1cm]{Images/Image_Eric_Chi_Cyg_Mai06.eps}
      \caption{ Couverture frequentielles (gauche) et images de
	$\chi$ Cyg (droite) obtenues à quatre phases stellaires
	différentes (de haut en bas : $\phi = 0,91$, 0,24, 0,67, et
	0,76). Ces images monttrent une nette variation à la fois en taille et en
	morphologie.   }
         \label{fig:Chi_Cyg_rec}
   \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{$\chi$ Cygni}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

$\chi$ Cygni est une étoile de la branche asymptotique des géantes. De
type Mira, elle présente de forte variations photométriques, avec une
période de 408 jours. Comme on peut nettement l'observer sur la
figure~\ref{fig:lum_cyg}, sa luminosité peut passer, en 200 jours, d'une
magnitude 3.5 à une magnitude 14 dans le visible, soit 1500 fois plus faible. Par
rapport aux autres étoile de la classe des Mira, elle a la
particularité d'être de type S, c'est-à-dire ayant une atmosphère très
carbonée, avec un ratio Oxygène sur Carbone d'environ 1. Ceci est la
conséquence d'un important ``dredge-up'' au cours duquel le phénomène
de convection a pu se produire suffisamment profondément dans l'étoile
pour que les métaux produits par la fusion au c\oe ur de l'étoile
puissent revenir à la surface. Pour autant, tout l'oxygène n'est pas
sous forme de monoxyde de carbone comme en témoigne la présence d'eau
ou même de masers SiO \citep{1999A&AS..139..461A}. Ceci s'explique en
partie par le type spectral qui passe périodiquement de S à M, au
maximum de luminosité.

Nous avons eu la chance de pouvoir observer $\chi$ Cyg au cours des 4
missions d'observation, ceci nous a permis d'avoir une image de l'étoile à
différentes phases. Les images obtenues à partir du logiciel de
reconstruction montrent d'ailleurs clairement des différences de
morphologies aux différentes époques
(figures~\ref{fig:Chi_Cyg_rec}). Les phases d'observations sont,
chronologiquement, 0,91, 0,24, 0,67 et 0.76. Les rayons observés
varient de 1 à 1,5 unité astronomique. Cette étoile est étudiée plus
en détails dans le chapitre~\ref{sec:temporelle}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{R leo}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


   \begin{figure}[h]
   \centering
   \includegraphics[width=6.2cm]{Images/UV_plane_Rleo.eps}
   \includegraphics[width=7cm]{Images/Image_Eric_Rleo.eps}
   \includegraphics[width=6.2cm]{Images/UV_plane_Rleo_Mars.eps}
   \includegraphics[width=7cm]{Images/Image_Eric_Rleo_mars.eps}
      \caption{ 
Plan $u$-$v$ et images de R leo obtenues au cours des observations de
mars ($\phi = 0,92$) et mai 2005 ($\phi = 0,05$).}
         \label{fig:Rleo_rec}
   \end{figure}

R leo est une étoile Mira des plus brillantes. Elle a été découverte
par J. A. Koch en 1782, après Mira (omicron Ceti), $\chi$ Cyg et R
Hydrae. Avec une période de 312 jours, cette étoile présente des
variations photométriques de plus de 5 magnitudes dans le visible
(figure~\ref{fig:lum_Rleo}).  Sa taille angulaire et sa luminosité en
ont fait un cas d'école dans l'étude à haute résolution angulaire des
Mira. Comme pour $\chi$ Cyg, de multiples techniques d'observations
ont été utilisées, comme l'occultation lunaire
\citep{1991A&A...249..397D}, l'interférometrie des tavelures
\citep{1977ApJ...218L..75L,2001A&A...376..518H} le masquage de pupille
\citep{2004MNRAS.349..303J} ou encore l'interférométrie longue base
\citep[][ont observé avec les interféromètres COAST,
IOTA/FLUOR, ISI,
VLTI/VINCI]{1998MNRAS.297..462B,1999A&A...345..221P,2003ApJ...589..976W,2004A&A...426..279P,2005A&A...431.1019F}.
Ces observations confirment une taille angulaire variable en fonction
de la longueur d'onde et la présence d'une couche moléculaire proche
de l'étoile. De plus, de nombreuses observations témoignent de fortes
asymétries.

Nous avons observé cette étoile lors de deux missions successives en
mars et mai 2006. Au cours de ces deux mois, la morphologie de cet
objet a varié considérablement, à la fois en terme de taille et de
structure (figure~\ref{fig:Rleo_rec}). L'étoile montre, de plus, un
flux important extérieur à la photosphère, que l'on ne trouvait pas
sur $\chi$ Cyg et encore moins sur Alpha Boo. La question reste
ouverte sur l'origine de ce flux. On pourrait considérer que la couche
moléculaire observée par spectro-interfemétrie
\citep{2004A&A...426..279P} est la source de ce flux. Cependant, il
possède aussi de nombreuses similitudes avec le flux observé sur Mira,
ce qui pousse à envisager un effet de distorsion du champ
gravitationnel dû à un compagnon.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Mira}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


   \begin{figure}[h!] \centering
   \includegraphics[width=6.2cm]{Images/UV_plane_Mira.eps}
   \includegraphics[width=7cm]{Images/Image_Eric_Mira.eps} 
\caption{
   Couverture fréquentielle et image de omicron Ceti obtenue via le
   logiciel de reconstruction en aveugle. La structure de l'étoile est
   profondément différente de celle des autres Miras, avec notamment
   la présence de deux composantes, comme si une atmosphère étendue de
   gaz chaud entourait une photosphère fortement asymétrique. Nous
   supposons que cela est dû à la présence de Mira B, située à 600
   mas au sud-ouest de l'étoile.  } \label{fig:Mira_rec} 
\end{figure}

   \begin{figure}[h!]
   \centering
   \includegraphics[width=12cm]{Images/MiraAB.eps}
      \caption{ Images en infrarouge moyen de Mira A et B obtenues à
      partir du télescope IRTF \citep{2001ApJ...556L..47M}. La croix indique
      la position de Mira B telle qu'observée par Hubble en 1997. On
      peut voir l'influence de l'attraction gravitationnelle exercé
      par Mira B sur la poussière circumstellaire à Mira A.}
         \label{fig:IRTF}
   \end{figure}



En 1596, David Fabricus a utilisé omicron Ceti comme référence de la
position de Mercure. Il a ainsi découvert la première étoile variable
de longue période. En 1642, omicron ceti a reçu son nom commun, Mira,
soit ``la merveilleuse''. Elle a, par la suite, donné son nom à
l'ensemble des étoiles ayant le même type de pulsation, les variables
Mira.

Mira se caractérise par les types spectraux M2-M7 III, et une période
de pulsation de 332 jours (figure~\ref{fig:lum_Mira}). Elle fût
récemment sur le devant de la scène scientifique suite à l'imagerie
par le satellite Hubble d'un compagnon proche
\citep{1997ApJ...482L.175K}. \`A une distance du soleil d'environ 130
parsecs, Mira AB est le complexe symbiotique le plus proche que l'on
connaisse. Les étoiles sont séparées d'environ 600 mas, orbitant avec
une période d'environ 500 ans \citep{2002ApJS..139..249P}. L'étoile
secondaire serait une naine blanche
\citep{1954ApJS....1...39J,2005ApJ...623L.137K} accrétant l'atmosphère
de l'étoile principale Mira A. De multiples observations dans
l'ultraviolet (Hubble et FUSE) ont permis de calculer un taux
d'accrétion de $2,5 \times 10^{12}$ M$_\odot$ par an
\citep{2006ApJ...649..410W}. Ce taux est très faible comparé à la
perte de masse de l'étoile principale, estimée à environ $10^{-7}$
M$_\odot$/ans \citep{1988ApJ...332..299B}.

Nous avons observé Mira A durant 5 nuits au cours du mois d'octobre
2005. Sa déclinaison étant proche de 0 degré, la synthèse d'ouverture
due à la rotation de la Terre nous a permis une couverture homogène
des fréquences spatiales. On note une structure de l'atmosphère
profondèment différente des trois étoiles précédemment observées. Deux
composantes sont clairement visibles sur l'image reconstruite
figure~\ref{fig:Mira_rec}. La première, d'environ 70\% du flux, est
centrale et allongée dans la direction Nord-Est. La seconde correspond
à une atmosphère étendue sur deux fois la taille de la composante
centrale. Elle est excentrée par rapport à la première dans la
direction de l'étoile Mira B (Sud-Est). Cette géométrie est
profondément différente de celle observée sur R-leo et $\chi$ Cyg. Il
semblerait donc s'agir de matière extraite de la géante par
l'influence gravitationnelle de l'étoile secondaire. Ce résultat est
en accord avec l'asymétrie de l'enveloppe de poussière observée en
infrarouge moyen avec le télescope IRTF (figure~\ref{fig:IRTF}).



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bételgeuse}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \begin{figure}[h]
   \centering
   \includegraphics[width=6.2cm]{Images/UV_plane_Betel.eps}
   \includegraphics[width=7cm]{Images/Image_Eric_Betel.eps}
      \caption{ Plan $u$-$v$ et imagerie en aveugle de Bételgeuse en
      octobre 2006. On peut distinguer une surface clairement
      inhomogéne pouvant faire penser aux surfaces convective simulés
      par Freytag (figure~\ref{fig:Freytag}). }
         \label{fig:Betel}
   \end{figure}



   \begin{figure}[h]
   \centering
   \includegraphics[width=10cm]{Images/Young.eps}
      \caption{ Imagerie paramétrique de Bételgeuse par \citet{2000MNRAS.315..635Y}. }
         \label{fig:Betel_Y}
   \end{figure}


La constellation d'Orion est l'une des plus connues, visible de
l'hémisphère Nord comme de l'hémisphère sud. Les deux étoiles les plus
brillantes, Rigel et Bételgeuse occupent respectivement les coins
Sud-Ouest et Nord-Est. Les premières mesures de variations de
luminosité de Bételgeuse ont été effectuées en 1836 par John
Hershel. Dans le visible, elle oscille entre des magnitudes allant de
0,2 à 1,2 (figure~\ref{fig:lum_betel}). \`A cette longueur d'onde, il
s'agit de la septième étoile la plus brillante de l'hémisphère
Nord. Cependant, comme toutes les géantes rouges, cette étoile émet
principalement dans le domaine de l'infrarouge, ce qui,
bolométriquement, en fait l'étoile la plus brillante du ciel. Ceci est
dû à sa distance (85 pc), mais surtout à sa taille, d'environ 630 fois
le diamètre de notre soleil \citep[$\theta_{\rm UD} \approx$ 43,3 mas
dans ][]{2004A&A...418..675P}.

C'est en 1920 qu'a eu lieu la première mesure de diamètre
stellaire. Elle a été effectuée sur Bételgeuse par Michelson, qui a
estimé son diamètre à environ 0,044 mas. Ceci en fait l'étoile la plus
grosse, en terme de taille angulaire. La plupart des instruments
d'interférométrie stellaire ont par conséquent étudié cet
objet. Utilisant la technique d'interférométrie des tavelures, Francois et
Claude Roddier ont été les premiers à reconstruire une image de la
surface stellaire \citep{1985ApJ...295L..21R}. Ils en ont déduit la
présence de poussières assombrissant le disque, créant une importante
asymétrie. Diverses observations de Bételgeuse s'en sont suivies
\citep{1997MNRAS.291..819W,2000MNRAS.315..635Y}. Toutes ont confirmé
l'existence d'asymétries et, notamment, de taches, parfois sombres ou
brillantes, sur la surface. \`A titre d'exemple, la
figure~\ref{fig:Betel_Y} montre les reconstructions auxquel 
\citet{2000MNRAS.315..635Y} ont abouti. Il s'agit dans ce cas de
l'imagerie paramétrique, c'est-à-dire qu'il ont ajusté une photosphère
à leurs données, à laquelle ils ont rajouté des taches.


Contrairement à eux, la précision que nous avons sur les visibilités,
ainsi que l'étendu de la couverture fréquentielle, nous a permis une
reconstruction en aveugle de la surface stellaire
(figure~\ref{fig:Betel}). L'ensemble est en accord avec les
prédictions de \citet{2003csss...12.1024F} concernant l'influence de
la convection sur l'atmosphère des super géantes, bien que l'image
observée diffère nettement d'un disque uniforme qui serait ponctué de
taches.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{$\mu$ Cep}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


   \begin{figure}[h]
   \centering
   \includegraphics[width=6.2cm]{Images/UV_plane_MuCep.eps}
   \includegraphics[width=7cm]{Images/Image_Eric_MuCep.eps}
      \caption{ Plan $u$-$v$ et imagerie en aveugle de $\mu$ Cep.}
         \label{fig:mu_cep_rec}
   \end{figure}


La variabilité de $\mu$ Cep a été découverte en 1848 par John
Russel. Il s'agit de l'une des étoiles les plus grosses du ciel après VV
Cephei et Epsilon Aurigae. $\mu$ Cep a de nombreux points communs avec
Bételgeuse. Il s'agit d'une supergeante semi-réguliaire (de type SRc)
avec des amplitudes de variations photométriques dans le visible
d'environ 1.5 magnitude (figure~\ref{fig:lum_mucep}). Son type
spectral est M2eIa, avec des périodes de pulsation de 730 et 4400
jours \citet{2006MNRAS.Kiss}.

Nous avons pu observer cet objet courant mai 2006 en utilisant le mode
dispersé d'IOTA (figure~\ref{fig:mu_cep_rec}). Outre sa taille remarquable, il est intéressant de
noter que la reconstruction nous donne un objet très uniforme, loin de
l'image obtenue de Bételgeuse. Ceci peut être tout simplement la
conséquence d'un manque de résolution. Cependant, on voit clairement
une asymétrie dans la structure de l'étoile.  Il est à noter que la
couche moléculaire, telle qu'observée par \citet{2005A&A...436..317P},
n'est pas visible dans cette image reconstruite. On verra dans le
paragraphe~\ref{sec:dispertion} qu'elle est tout de même présente dans
nos données, et que nous pouvons la mettre en évidence par imagerie
paramétrique.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{CH Cyg}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \begin{figure}[h]
   \centering
   \includegraphics[width=6.2cm]{Images/UV_plane_CHCyg.eps}
   \includegraphics[width=7cm]{Images/Image_Eric_CH_Cyg.eps}
      \caption{ Plan $u$-$v$ et imagerie en aveugle de CH Cyg.}
         \label{fig:ch_cyg}
   \end{figure}

A l'instar de Mira, CH Cyg est une étoile variable
symbiotique. L'aspect particulier de son spectre a longtemps intrigué
les chercheurs. En effet, à chaque type d'étoile correspond une lettre
(de A à M) distribuée en fonction de l'importance de la raie
d'hydrogène et d'hélium. Toujours utilisée, cette classification a été
ré-arrangée afin de classer les étoiles par ordre croissant de
température (OBAFGKM). Cependant, certaines étoiles, dont CH Cyg, ne
trouvent pas de place dans cette classification. CH Cyg possède, en
effet, une température proche de celle du type M, mais avec des raies
en émission typiques des étoiles de type O.

Nous avons retenu l'idée selon laquelle CH Cyg est constituée de deux
étoiles. La première est une géante rouge et la deuxième une naine
blanche accrétant l'atmosphère de la première
\citep{1990A&A...235..219M}. Cette hypothèse est, par ailleurs,
corroborée par la courbe de lumière de l'étoile qui présente à la fois
des oscillations périodiques et d'importantes éruptions (comme celle
observée en 1986 ; cf figure~\ref{fig:lum_ch}). L'existence d'un compagnon
accrétant de la matière est confirmée par la présence de jets
observables dans le domaine de longueur d'onde radio
\citep{2001MNRAS.326..781C} et X
\citep{2004ApJ...613L..61G}. Actuellement, les astronomes s'accordent
sur la présence d'un système triple \citep{1993AJ....105.1074H}. Il
serait composé d'une naine blanche entourée d'un disque d'accrétion
orbitant avec une période de 2,07 ans autour d'une géante
semi-régulière de type M7 III. Autour de ce système en interaction
graviterait, avec une période de 14,5 ans, une troisième étoile
appartenant à la séquence principale (naine G-K).

Nous avons pu observer cette étoile durant deux nuits. La couverture
du domaine fréquentiel (figure~\ref{fig:ch_cyg}) est par
conséquent très diluée. Du fait de la petit taille angulaire de
l'étoile, et cela, même en utilisant la base maximale de
l'interféromètre IOTA (38 mètres), nous n'avons pas pu atteindre le
deuxième lobe de la courbe de visibilité. Nous avons, cependant,
constaté des clôtures de phase de l'ordre de la dizaine de degrés,
démontrant la présence d'asymétries. La résolution limitée, ainsi que
la faible quantité de données, ne nous ont pas permis de caractériser
cette asymétrie.


   \begin{figure}
   \centering
   \includegraphics[width=12cm]{Images/chi_cyg.eps}
   \includegraphics[width=12cm]{Images/R_leo.eps}
   \includegraphics[width=12cm]{Images/Mira.eps}
      \caption{Courbe de lumière correspondant au complexe symbiotique
      Mira AB. La pulsation de l'étoile post-AGB Mira A est clairement
      visible avec une période de 332 jours. Les modulations à plus
      grande période (environ 14 ans) sont interprétées comme des
      variations de l'accrétion dues à Mira B.}
         \label{fig:lum_Mira}
         \label{fig:lum_Rleo}
         \label{fig:lum_cyg}
   \end{figure}

   \begin{figure}
   \centering
   \includegraphics[width=12cm]{Images/betel.eps}
   \includegraphics[width=12cm]{Images/Mu_cep.eps}
   \includegraphics[width=12cm]{Images/CH_Cyg.eps}
      \caption{Courbe de lumière de Bételgeuse extraite du site de l'American
      Association of variable star observers.}
         \label{fig:lum_ch}
         \label{fig:lum_mucep}
         \label{fig:lum_betel}
   \end{figure}

==> iota.tex <==
\newpage

\section{L'observatoire}

\section{L'instrument}

\section{La mesure}

\subsection{La visibilité}

\subsubsection{Visibilité dans le cas général}

\subsubsection{Visibilité d'un disque uniforme}

\subsubsection{Visibilité d'un object centrosymétrique}

\subsection{La cloture de phase}

\subsubsection{Le principe}

\subsubsection{Quelques cas particuliers}

==> realisation_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Il  existe deux types de paramètres entrant en jeu lors de la conception
de l'instrument. Un certain nombre d'entre eux sont liés à
l'environement de l'instrument et ne peuvent être modifiés. Il s'agit
de :
\begin{itemize}
\item $D$, le diamètre du télescope
\item $r_0$, le diamètre d'une surface cohérente ($\sigma < 1$ rad) du
  front d'onde incident perturbé par la turbulence atmosphérique. Pour
  un système comprennant une optique adaptative, nous
  utiliserons à la place de $r_0$ le paramètre de
  Fried généralisé $\rho_0$ \citep{2000JOSAA..17..903C}.
\item Les bruits de photons et de détecteur. 
\end{itemize}
Ensuite, en fonction de ceux-ci, il faut choisir un certain nombre de
paramètres physiques optimisant les performances finales. Ces
paramètres libres sont :
\begin{itemize}
\item $M$, le nombre de sous-pupilles et de fibres optiques
\item $d$, la taille des sous-pupilles
\item $\eta$, le rapport entre l'ouverture numérique des lentilles et
  celle des fibres
\item $\Delta \lambda/\lambda_0$ la bande passante spectrale
\item $D'/d'$, le rapport maximal de taille entre la sous-pupille de sortie et la
  distance séparant deux sous-pupilles.
\end{itemize}
Il s'agit de simuler l'influence de chacune de ces valeurs
dans le cadre des paramètres fixes. Par exemple, le diamètre du
télescope contraint le nombre de sous-pupilles par la relation :
\begin{equation}
D \leq \sqrt{M} d \,.
\end{equation}
Cependant, ces paramètres influent sur différents facteurs. Nous nous
focaliserons au cours de ce chapitre sur la sensibilité de
l'instrument et les sources d'erreurs sur les visibilités (voir
tableau~\ref{tb:choix} ci-dessous).


\begin{table}[h]
\caption{Influence des caractéristiques de l'instrument}
\label{tb:choix}
\centering
\begin{tabular}{lccccc}
\hline
\hline
& $d$ & $\eta$ & $\Delta \lambda/\lambda_0$ & $D'/d'$ & Paragraphe\\
\hline
Champ de la fibre & \checkmark & \checkmark & &&\ref{sc:champ_fibre} \\
Bruit de confusion & \checkmark & \checkmark & &&\ref{sc:confusion} \\
Champ de l'interféromètre & & & \checkmark &\checkmark & 
\ref{sc:Champ_interfero}  \\
Bruit de piston & & & \checkmark & \checkmark & \ref{sc:piston} \\
Sensibilité  & \checkmark & \checkmark & \checkmark & \checkmark &  \\
\hline
\end{tabular}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{L'injection dans les fibres monomodes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{sc:inject}

\subsection{Eléments théoriques}


   \begin{figure}[h!]
   \centering
   \includegraphics[width=10cm]{Images/Fibre.eps}
   \caption{ Flux en sortie de fibre. La diffraction crée un champ
   divergeant, quasi-Gaussien. Il peut être caractérisé par une
   largeur fixé par un seuil de 5\% ($1/e^2$) ou de 13,5\%
   ($1/e$). Dans le c\oe ur de la fibre, le champ est défini par le
   diamètre modal $w_O$. L'ouverture numérique correspond un angle que
   nous définirons au cours de cette thèse par le niveau d'intensité
   de 5\%.  }
         \label{fig:mesure_ON}
   \end{figure}

Certain paramètres fondamentaux caractérisent les fibre optiques
monomodes. Ils sont déterminé par la physique de la fibre et servent
de référence lors de l'achat ces fibres. Il s'agit de :
\begin{itemize}
\item L'ouverture numérique $ON$, angle dû à la diffraction de la
  lumière à la sortie de la fibre. Cette valeur est achromatique.
  Dans le cas d'une fibre à saut d'indices, elle est fixée par
  l'indice de la fibre et de son c\oe ur: $ON =
  \sqrt{n_c^2-n_g^2}$. Cette valeur est importante car elle peut être
  déterminée expérimentalement (figure~\ref{fig:mesure_ON}).
\item Le diamètre du mode fondamental $w_0$ (en anglais, MFD pour Mode
  Field Diameter) est une longueur chromatique et ne correspond pas
  nécessairement au diamètre du coeur. Alors que l'ouverture numérique
  est définie par un seuil d'intensité de 5\%, le diamètre est
  caractérisé par le seuil de 13,5\%. La relation entre ces deux
  valeurs est la suivante :
\begin{equation}
w_0=\frac{\sqrt{6}}{\pi} \frac{ \lambda}{ON}\,.
\label{eq:w0_ON}
\end{equation}
\item La fréquence de coupure $\lambda_c$. Il s'agit de la limite
  spectrale pour que la fibre se comporte comme une fibre
  monomode. Aux longueurs d'ondes inférieures, d'autres modes
  apparaissent. L'utilisation d'une fibre monomode se fait
  généralement dans le domaine spectral $\lambda_c < \lambda < 1,3
  \lambda_c$. Aux longueurs d'ondes supérieures, la fibre devient
  sensible aux courbures et le facteur de transmission
  décroit. $\lambda_c$ est relié à l'ouverture numérique et au rayon
  du c\oe ur
  de la fibre ($a$) par la relation:
\begin{equation}
\lambda_c=\frac{2 \pi a ON}{2,405} \,.
\end{equation}
\end{itemize}

Le champ dans la fibre est radial, avec une amplitude proche d'une
fonction Gaussienne. Cette approximation donne :
\begin{equation}
E(r) \propto  \exp\left(\frac{-4r^2}{w_0^2}\right)\,.
\end{equation}
Dans un plan image fictif définit par une focale $f$, le champ en  coordonnées angulaires
donne :
\begin{equation}
E_\bullet(x,y) \propto \exp\left(-\frac{4(x^2+y^2)}{w_0^2}\right)\,.
\end{equation}
Nous pouvons alors utiliser la
transformée de Fourier qui lie le champ dans le plan
pupille au champ du plan focal\footnote{d'après la diffraction de
Fraunhoffer, la transformé de Fourier du champ pupillaire est égale à
la tranformé de Fourier du champ focal : $E_\bullet(\alpha,\beta) \propto
TF(E_\circ(U,V))$. Dans cette formule, $\alpha$ et $\beta$
correspondent à la position angulaire ($x/f$; $f$ la distance focale
et $x$ la position dans le plan focal), et $U$ et $V$ sont des
distances en unités de longueur d'onde ($u/\lambda$; $u$ la position
dans le plan pupille).} :
\begin{equation}
E_\circ(u/\lambda,v/\lambda) \propto TF^{-1}(E_\bullet(x/f,x/f))
\label{eq:tfh}
\end{equation}
pour en déduire le champ pupillaire associé au mode fondamental de la
fibre:
\begin{equation}
E_\circ(u,v) \propto
\exp\left(-\frac{\pi^2 w_0^2(u^2+v^2)}{4f^2\lambda^2}\right) \, .
\end{equation}
qui peut également s'écrire d'après l'équation~\ref{eq:w0_ON}:
\begin{equation}
E_\circ(u,v) \propto
\exp\left(-\frac{3 (u^2+v^2)}{2f^2\,ON^2}\right) \, 
\label{eq:champ_fibre}
\end{equation}
Il est intéressant de noter que l'amplitude du champ dans la
pupille est une Gaussienne indépendante de la longeur d'onde,
d'écart type $f^2\,ON^2/3$.

\subsection{L'efficacité de couplage}

L'amplitude complexe couplée dans la fibre est le produit scalaire
normalisé du mode fondamental de la fibre ($E$) par le champ électrique
incident ($U$):
\begin{equation}
A =
\frac{ \iint_{-\infty}^{+\infty}
  U_\bullet(x,y)\,.\,E_\bullet^\star(x,y)\ dx
  dy}{\iint_{-\infty}^{+\infty}
  |U_\bullet(x,y)|^2 dx
  dy\,\times\,\iint_{-\infty}^{+\infty}
  |E_\bullet(x,y)|^2dx dy} \,.
\end{equation}
Elle peut être calculée de la même façon par le recouvrement des champs
dans le plan pupille (théorème de Parceval):
\begin{equation}
A =
\frac{\iint_{-\infty}^{+\infty} U_\circ(u,v)\,.\,E^\star_\circ(u,v)\
  dudv}{\iint_{-\infty}^{+\infty}|U_\circ(u,v)|^2 dudv\,\times\,\iint_{-\infty}^{+\infty}|E_\circ(u,v)|^2dudv} \,.
\end{equation}
L'efficacité de couplage correspond à l'énergie injectée dans la fibre
par rapport à l'énergie totale incidente. Elle est égale au carré du
module de l'amplitude complexe :
\begin{equation}
\rho = |A|^2 \,.
\end{equation}

L'équation du champ de la fibre dans le plan pupille a été établie en
équation~\ref{eq:champ_fibre}. En faisant intervenir le diamètre de la
sous-pupille ($d$) et le rapport d'ouverture numérique entre la lentille
d'injection et la fibre ($\eta=ON_{\rm lentille} / ON_{\rm fibre}$),
on peut obtenir une forme simple, normalisée :
\begin{equation}
E_\circ(u,v) = \frac{ 2 \eta}{ d} \sqrt{ \frac{3}{\pi}} 
\exp\left(-6 \frac{ (u^2+v^2)}{d^2} \eta^2 \right) \, ,
\end{equation}
où $u$, $v$ et $d$ sont respectivement les coordonnées dans le plan
pupille et le diamètre de la sous-pupille. 

%Le champ provenant de l'objet astrophysique est plus complexe à
%obtenir, car dépendant des turbulence atmosphérique. 

\subsection{Injection dans le cas d'un front d'onde cohérent}


   \begin{figure}[h]
   \centering
\resizebox{\hsize}{!}{
   \includegraphics{Images/Efficacite_sans_pertub.eps}
   \includegraphics{Images/Champ_sans_pertub.eps}}
   \caption{ A gauche : Efficacité de couplage en fonction du rapport
   d'ouverture $\eta = ON_{\rm lentille} / ON_{\rm fibre}$. Dans le
   cas d'un front d'onde incident cohérent, l'efficacité de couplage
   est maximale pour $\eta =0,92$. A droite : le champ électrique
   associé à la fibre et à l'onde incidente dans le plan pupille.
}
         \label{fig:champ_fibre}
   \end{figure}


Pour une pupille pleine, et en l'abscence de perturbations
atmosphériques, le champ provenant de l'objet astrophysique s'écrit de
façon normalisé :
\begin{eqnarray}
U_\circ(u,v) = &  \frac{2}{\sqrt{\pi} d}  & {\rm si}\ \sqrt{u^2+v^2} \leq
d/2 \\ & 0 & {\rm sinon}.
\end{eqnarray}
D'où l'amplitude complexe de couplage :
\begin{equation}
A = \iint_{\sqrt{u^2+v^2} \leq d/2}  \frac{4\sqrt{3} \eta }{\pi
  d^2} 
\exp\left(-6 \frac{ (u^2+v^2)}{d^2} \eta^2 \right)       dudv \,,
\end{equation}
et :
\begin{equation}
A = \frac{2}{\sqrt{3} \eta} \left( 1 -\exp\left(-\frac{3 \eta^2}{2}\right)\right)  \,.
\end{equation}
Par conséquent, l'efficacité de couplage s'écrit :
\begin{equation}
\rho = \frac{4}{3  \eta^2} \left(1 -\exp\left(-\frac{3 \eta^2}{2}\right)\right)^2  \,.
\end{equation}
avec un maximum pour $\eta = 0,92$ et une efficacité de couplage de
81 \%.

\subsection{Sensibilité dans le cas d'un front d'onde perturbé}

   \begin{figure}[h]
   \centering
\resizebox{\hsize}{!}{
   \includegraphics{Images/Energie_couple.eps}
   \includegraphics{Images/eta_max.eps}}
   \caption{ A gauche : $\rho d^2$, une quantité proportionnelle à
     l'énergie injectée dans une fibre. Pour une petite pupille
     l'énergie injectée est maximale pour $\eta=0,92$. Lorsque la
     taille de la pupille augmente, le $\eta$ maximisant l'énergie
     couplée change. Nous l'avons représenté sur la courbe de droite,
     et approximé par la relation : $\eta = d/r_0*0.115+0.92$ (courbe
     en pointillés).  }
         \label{fig:inject_turb}
   \end{figure}

En considérant le bruit du détecteur, la sensibilité de l'instrument
est liée au nombre de photons reçu par pixel, et non à celui de
l'ensemble de la pupille. Plus exactement, à nombre de photons fixe,
plus on utilise de fibres, plus la sensibilié décroit.

Ainsi, une caractérisation de la sensibilité peut être obtenue à
partir de l'énergie couplée en moyenne dans une fibre. Cette énergie
est proportionnelle à l'efficacité de couplage et à l'aire de la
sous-pupille. Dans le cas d'un front d'onde incident parfaitement
cohérent, la sensibilité maximale est obtenue pour $\eta= 0,92$ et un
diamètre de sous-pupille maximal. Lorsque le front d'onde est perturbé
par l'atmosphère, la sensibilité maximale n'est plus obtenue pour une
valeur unique de $\eta$. Nous avons utilisé un logiciel de simulation
de fronts d'ondes perturbés pour en déduire une moyenne de
l'efficacité de couplage en fonction du rapport $d/r_0$. La thèse
d'\citet{Assemat:PhD} décrit ce logiciel en détails.

Nos résultats montrent que l'augmentation de la taille de la pupille
n'entraîne pas obligatoirement une augmentation notable de l'énergie
injectée. A $r_0$ fixé, l'énergie est proportionnelle à $\rho
d^2$. Nous avons représenté cette valeur en fonction de $d$ sur le
graphique de gauche de la figure~\ref{fig:inject_turb} ($d$ est donné
en facteur de $r_0$). La courbe rouge représente la valeur optimale en
l'abscence de perturbation ($\eta =0,92$). Les autres courbes
correspondent à différentes valeurs de $\eta$ comprises entre 0,9 et
1,5. Un certain nombre de conclusions peuvent en être tiré :
\begin{itemize}
\item Lorsque $d/r_0 < 2$, le choix du facteur de couplage n'est pas
  déterminant si $0,9 < \eta < 1,5$.
\item L'efficacité de couplage optimale est obtenue pour une ouverture
  numérique de la fibre plus faible, que l'on peut trouver à partir de
  la loi affine suivante :
\begin{equation}
\eta = \frac{ON_{\rm lentille}}{ON_{\rm fibre}} = d/r_0*0.115+0.92 \,.
\end{equation}
\item Lorsque $d/r_0 > 3$, l'énergie injectée n'augmente plus que
marginalement.
\end{itemize}

{\bf A la lumière de ces résultats, une valeur optimale en terme de
sensibilité est obtenue pour une taille de sous-pupille $d = 3 r_0$ et un
rapport d'ouvertures numériques $\eta =1,25$.}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Champ et phénomène de confusion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

La résolution de l'instrument est fixée par le diamètre $D$ de la
pupille totale du télescope. Le nombre d'éléments de résolution est
déterminé par le champ observé sur le ciel. Celui-ci s'obtient par un
calcul d'efficacité de couplage similaire à celui effectué dans la
section précédente.


\subsection{Champ dans le cas d'un front d'onde cohérent}
\label{sc:champ_fibre}

\begin{figure}
   \centering
\resizebox{\hsize}{!}{
   \includegraphics{Images/Champ1.eps}
   \includegraphics{Images/Energy_eta.eps}}
   \caption{ A gauche : efficacité de couplage en fonction de la
   position de l'étoile dans le ciel, en l'absence de
   perturbations. Le champ injecté dans la fibre est en unités
   de $\lambda/d$, et peut ainsi être aisément comparé à l'élément de
   résolution de l'instrument qui est de $\lambda/D$. A droite :
   l'énergie couplée en fonction du paramètre $\eta$. Lorsque ce
   paramètre augmente, le champ augmente. Cependant, passé une valeur
   optimale, l'accroissement de $\eta$ se traduit également par une
   diminution du flux couplé dans la fibre.}
   \label{fig:Champ}
\end{figure}

Lorsque l'objet observé n'est plus sur l'axe du télescope, le champ
incident est ``tilté'' par rapport au champ de la
fibre. L'efficacité de couplage pour une source hors axe définie ainsi
le champ de la fibre. Pour une source distante d'un angle $\alpha$ de
l'axe du système, on obtient l'expression suivante du champ :
\begin{eqnarray}
U_\circ(u,v) = &  \frac{\exp(-2 \I \pi u \alpha)}{\sqrt{\pi} (d/2)}  & {\rm si}\ \sqrt{u^2+v^2} \leq
d/2 \\ & 0 & {\rm sinon},
\end{eqnarray}
et une efficacité de couplage :
\begin{equation}
\rho = \left| \iint_{\sqrt{u^2+v^2} \leq d/2}  \frac{4\sqrt{3} \eta \exp(-2 \I \pi u \alpha)}{\pi
  d^2} 
\exp\left(-6 \frac{ (u^2+v^2)}{d^2} \eta^2
  \right)       dudv \right|^2\,,
\label{eq:conf}
\end{equation}
La figure~\ref{fig:Champ} représente le champ pour différentes valeurs
de $\eta$. Celui-ci est fortement limité par l'injection dans la
fibre. Par exemple, pour un télescope de diamètre $D=7d$, l'élement de
résolution est de $\lambda/7d$. Or, pour $\eta=0,92$, nous avons un
champ total à mi-hauteur de $0,6\lambda/d$. Il n'est alors composé que
de 4 éléments de résolutions. C'est pourquoi il est préférable de
choisir $\eta$ aussi grand que possible.  Pour pouvoir décider d'un
compromis entre champ et flux injecté, nous avons représenté ces
valeurs dans la partie de droite de la figure~\ref{fig:Champ}.

\subsection{Le bruit de confusion}
\label{sc:confusion}

\begin{figure}[h]
   \centering
\resizebox{\hsize}{!}{
   \includegraphics{Images/Champ2.eps}
   \includegraphics{Images/Champ3.eps}
   \includegraphics{Images/Champ4.eps}}
\resizebox{\hsize}{!}{
   \includegraphics{Images/Champ5.eps}
   \includegraphics{Images/Champ6.eps}
   \includegraphics{Images/Champ7.eps}}
   \caption{ Partie supérieure : champ de vue moyen de l'instrument en
   présence de turbulences. Trois cas sont étudiés où $d=r_0$, $2r_0$
   et $3r_0$.  Partie inférieure : écart d'injection entre le champ
   théorique d'une fibre (figure~\ref{fig:Champ}) et en présence de
   turbulences. On peut noter une zone critique (entre 1 et 2
   $\lambda/d$) où la présence d'un objet introduirait un bruit de
   confusion important.}
   \label{fig:Champs}
\end{figure}

Le bruit de confusion est également un paramètre qui doit entrer en
jeu lors de la caractérisation de l'instrument. Ce bruit correspond à
l'influence de la turbulence sur le champ de vue des fibres. Le tip et le
tilt atmosphériques, notamment, font que les fibres ne ``regardent'' pas
toutes nécessairement dans la même direction. La visibilité alors
mesurée peut ainsi être faussée.  A ce titre, l'observation d'un système binaire
peut s'avérer problématique si le flux injecté dans les fibres ne
provient pas simultanément des deux objets.

Pour mesurer cet effet, nous avons utilisé l'équation~\ref{eq:conf} à
laquelle nous avons ajouté la présence de perturbations
atmosphériques. Nous en avons déduit le champ de vue moyen des fibres
en présence de turbulences. Les résultats sont présentés
figure~\ref{fig:Champs} pour trois tailles de sous-pupille: $r_0$,
$2r_0$ et $3r_0$. Sans surprise, la présence de turbulence augmente le
champ, d'un facteur pouvant aller jusqu'à trois dans le cas
$d=3r_0$. La différence entre le champ d'une fibre sans et avec
turbulence est représentée dans les trois graphiques du bas de la
figure~\ref{fig:Champs}. Ceux-ci révèlent clairement un espace du champ
(entre 1 et 2 $\lambda/d$) où la présence d'un objet introduirait une
source d'erreur dans la mesure des visibilités. Cependant, il n'est
pas aisé d'en déduire un critère pour estimer l'influence de ce flux
sur les visibilités générées par l'algorithme itératif du Chapitre
3. Nous pouvons néanmoins retirer de cette étude que le bruit de
confusion diminue lorsque $\eta$ augmente, ou lorsque le rapport
$d/r_0$ diminue.

{\bf En conclusion, et en considérant la taille d'une sous-pupille
choisie de façon à maximiser la sensibilité de l'instrument, il est
préférable de choisir un $\eta$ le plus élevé possible afin de
maximiser le champ et de minimiser le bruit de confusion. Au regard de
la figure~\ref{fig:Champ}, un bon compromis existe pour $d=3r_0$ et
$\eta = 1,5$.}

%\clearpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Recombinaison et bande spectrale}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{La modulation spatiale en monochromatique}

\begin{figure}[h]
   \centering
\resizebox{\hsize}{!}{
   \includegraphics{Images/Recombinaison.eps}}
   \caption{Schéma d'un systéme de recombinaison à deux faisceaux}
   \label{fig:schema_pup_s}
\end{figure}


Le champ électrique dans la pupille de sortie est composé du champ
sortant de chacune des fibres optiques. Pour effectuer une analyse détaillée de
l'influence du mode de recombinaison, nous avons travaillé sur un
système simple de recombinaison à deux faisceaux.  Le schéma de la
figure~\ref{fig:schema_pup_s} représente un tel système. Les
paramètres physiques entrant en jeu dans la recombinaison sont : 
\begin{itemize}
\item $d'$, le diamètre d'un faisceau de sortie défini tel que :
  $d'=2 f\,ON$
\item $D'$, la distance séparant les deux faisceaux dans le plan
  pupille
\item $f'$ la focale de la lentille de recombinaison. Cette focale
  intervient dans le calcul de la largeur de la tache de
  diffraction. Nous nous sommes affranchi de cette valeur par
  l'utilisation des coordonnées angulaires du plan focal ($\alpha=x/f'$
  et $\beta=y/f'$)
\end{itemize} 
Interviennent également le champ transmis par chacune des fibres
($g_1$ et $g_2$) et leur déphasage ($\Delta \phi$). A partir de
l'équation~\ref{eq:champ_fibre}, nous avons déduit le champ dans la
pupille de recombinaison :
\begin{equation}
E_{1\circ}(u,v) \propto g_1
\exp\left(-\frac{6  (u^2+v^2)}{d'^2}\right) * \delta(u+D'/2)
\end{equation}
pour le premier faisceau, et pour le second :
\begin{equation}
E_{2\circ}(u,v) \propto g_2
\exp\left(\I\Delta \phi-\frac{6  (u^2+v^2)}{d'^2}\right) * \delta(u-D'/2)\,.
\end{equation}
La transformé de Fourier (relation~\ref{eq:tfh}) nous donne le champ
dans le plan focal, soit
\begin{equation}
E_{1\bullet}(\alpha,\beta) \propto g_1 
\exp\left(-\frac{\pi^2 d'^2 \lambda^2 (\alpha^2+\beta^2)}{6}\right) \exp(-\I\pi
D' \lambda\alpha )\,,
\end{equation}
et
\begin{equation}
E_{2\bullet}(\alpha,\beta) \propto g_2 
\exp\left(-\frac{\pi^2 d'^2\lambda^2
  (\alpha^2+\beta^2)}{6}\right) \exp(\I\Delta \phi +  \I\pi
D'\lambda\alpha)\,,
\end{equation}


L'image obtenue sur le détecteur correspond à l'énergie des champs
électriques des deux fibres. S'ils sont cohérents (source ponctuelle),
ils s'additionnent de manière complexe, s'ils ne le sont pas, ce sont
les valeurs absolues qui s'additionnent.  Dans la suite de ce
raisonnement, nous supposerons une source ponctuelle, cohérente
($V(u,v) =1$). Ainsi :
\begin{equation}
I(\alpha,\beta)=\left|E_{1\bullet}(\alpha,\beta)+E_{2\bullet}(\alpha,\beta)\right|^2\,
\end{equation}
nous donne :
\begin{equation}
I(\alpha,\beta) \propto  \left|g_1 \exp(-\I\pi D'\lambda\alpha) +g_2\exp(\I\Delta
\phi +\I\pi D'\lambda\alpha) \right|^2
\exp\left(-\frac{\pi^2 d'^2\lambda
  (\alpha^2+\beta^2)}{3}\right) \,.
\end{equation}
Et, en développant, nous arrivons alors à l'expression suivante :
\begin{equation}
I(\alpha,\beta) \propto \left(
g_1^2+g_2^2+2g_1g_2\cos(2\pi D'\lambda\alpha+\Delta\phi) \right)
\exp\left(-\frac{\pi^2 d'^2\lambda
  (\alpha^2+\beta^2)}{3}\right)\,.
\label{eq:image}
\end{equation}
Deux termes importants caractérisent l'image sur le détecteur. Le
premier correspond à la modulation dans laquelle réside
l'information sur la cohérence et la phase des franges.  Le deuxième
terme correspond à l'enveloppe de l'image. Il s'agit d'une Gaussienne
qui est l'image des c\oe urs des fibres optiques projetés
sur le détecteur.  Alors que la largeur de cette Gaussienne dépend de
la taille de la sous-pupille de sortie $d'$, la fréquence de
modulation des franges dépend de l'écart entre deux sous-pupilles
$D'$. Pour une fréquence d'échantillonage suffisante ($D'>2d'$), il
est tout à fait possible, au bruit de photons et de détecteur près, de
mesurer avec précision l'amplitude et la phase des franges. Cela change
lorsque l'on considère l'aspect chromatique de la lumière.


\subsection{L'influence de la bande spectrale}
\label{sc:inf_spect}

\begin{figure}[h]
   \centering
   \includegraphics[width=11cm]{Images/These_chrom.eps}
   \caption{ Influence du chromatisme sur les franges. A gauche :
   franges achromatiques. La longueur de cohérence est infinie et les
   franges sont présentes sur la totalité de l'image. A droite : le
   chromatisme entraine la modulation des franges par une fonction en
   sinus cardinal.}
   \label{fig:chrom}
\end{figure}

Même si l'objet astrophysique observé est achromatique, l'image
obtenue est, quant à elle, chromatique. Elle correspond à la somme des
images aux différentes longueurs d'ondes. Pour une bande spectrale
$\Delta\lambda$, on obtient par conséquent :
\begin{equation}
I(\alpha,\beta) =
\int_{\lambda_0-\Delta\lambda/2}^{\lambda_0+\Delta\lambda/2}
I(\alpha,\beta,\lambda) d\lambda \,,
\end{equation}
où $\lambda_0$ correspond à la longueur d'onde centrale. Cependant,
avant d'entreprendre l'intégration, il est important d'étudier
l'aspect chromatique du déphasage entre le champ des deux fibres
optiques. Plus exactement, puisque le piston, en unité de longueur,
est achromatique, le déphasage est proportionnel à la longueur
d'onde. Nous pouvons alors obtenir un terme de déphasage achromatique
($\delta \phi_0$) en effectuant le changement de variable suivant :
\begin{equation}
\Delta\phi=\Delta\phi_0\frac{\lambda}{\lambda_0}.
\end{equation}
Ainsi, l'aspect chromatique de l'image observée apparaît entièrement
lorsqu'elle est écrite sous la forme :
\begin{equation}
I(\alpha,\beta,\lambda) = S(\lambda) \left(
g_1^2+g_2^2+2g_1g_2\cos\left(\pi
D'\lambda\alpha+\frac{\lambda}{\lambda_0}\Delta\phi_0\right) \right) \exp\left(-\frac{\pi^2
d'^2 \lambda^2 (\alpha^2+\beta^2)}{3}\right)\,.
\label{eq:image_c}
\end{equation}

 L'influence de la longueur d'onde est multiple:
\begin{itemize}
\item L'objet ayant une certaine ``couleur'', celle-ci induit un terme
  de proportionalité chromatique $S(\lambda)$. Dans le cas d'une
  étoile de température 6000\,K observé dans les longueurs d'ondes du
  visible, le terme $S(\lambda)$ est à peu près constant
  constant. Cette hypothése sera utilisé par la suite.
\item L'enveloppe est également modifiée par le chromatisme. L'écart
  type de la Gaussienne diminuant avec la longueur d'onde. Par souci
  de simplification, nous négligerons l'influence chromatique de
  l'enveloppe et nous l'approximerons par une valeur moyenne:
  $\exp\left(-\frac{1}{3}\pi^2 d'^2 \lambda_0^2
  (\alpha^2+\beta^2)\right)$.
\item Le terme de modulation sera lui aussi affecté par la
  superposition de franges aux différentes fréquences. Ce phénomène
  crée une perte de la cohérence moyenne (voir
  figure~\ref{fig:chrom}).
\end{itemize}
 
De manière à établir l'influence du chromatisme sur le terme de
modulation, nous l'avons isolé avant de l'intégrer sur la longueur
d'onde. Ceci est possible dans l'hypothése où l'on néglige le
chromatisme de l'objet astrophysique et celui de l'enveloppe
Gaussienne :
\begin{eqnarray}
\label{eq:mod}
m(\alpha)&= &\int_{\lambda_0-\Delta\lambda/2}^{\lambda_0+\Delta\lambda/2} 
2g_1g_2\cos\left(2\pi
D'\lambda\alpha+\frac{\lambda}{\lambda_0}\Delta\phi_0\right) d\lambda \\
&=&2g_1g_2 \Delta\lambda/\lambda
{\rm \ sinc}\left(\pi D' \Delta\lambda\alpha +
\frac{\Delta\lambda}{2\lambda_0}\Delta\phi_0\right)
\cos(2\pi D' \lambda_0\alpha + \Delta \phi_0)
\,.
\end{eqnarray} 
Il apparaît deux composantes : une modulation achromatique $\cos(2\pi
D'\lambda_0 \alpha + \Delta \phi_0)$ à haute fréquence, et un sinus
cardinal à plus basse fréquence ($D' \Delta \lambda/2$). Ce dernier se
traduit par une perte de cohérence lorsque l'on s'éloigne de la
différence de marche optique nulle ($\Delta\phi_0 >> 0$). Si cette perte de cohérence était
constante, elle pourrait être calibrée et ne poserait pas de
problème. Cependant, lorsqu'elle est multipliée par l'enveloppe
Gaussienne de la fibre, la présence d'un piston ($\Delta\phi_0$) crée
des variations de la mesure de cohérence.


L'influence du chromatisme sur le facteur de cohérence est complexe et
dépend du mode de mesure de la cohérence.  Sur l'interféromètre IOTA
par exemple, la mesure de la cohérence est obtenue par la puissance
contenue dans le pic frange du domaine spectral. A l'opposé,
l'instrument AMBER du VLTI mesure une visibilité complexe par
l'ajustement de franges dans le domaine spatial. Dans notre cas, et
parce qu'il s'agit d'obtenir des valeurs complexes, il semble
préférable d'utiliser l'ajustement d'un cosinus en $\cos(2\pi D'
\alpha + \phi)$. Alors, une approximation de la cohérence
mesurée sera proportionnelle à l'enveloppe des franges intégrée sur le
détecteur. On obtient ainsi l'efficacité interférométrique $\mu$ :
\begin{equation}
\mu \propto \int_\infty {\rm sinc}\left(\pi D' \Delta\lambda \alpha +
\frac{\Delta\lambda}{2\lambda_0}\Delta\phi_0\right) \exp\left(-\frac{\pi^2 d'^2\lambda_0^2
  \alpha^2}{3}\right) d\alpha \,,
\end{equation}
ou bien, après le changement de variable $\nu = d'\lambda_0\alpha$ :
\begin{equation}
\mu \propto \int_\infty {\rm
sinc}\left(\frac{\Delta\lambda}{2\lambda_0}(2\pi \frac{D'}{d'} \nu +
\Delta\phi_0)\right) \exp\left(-\frac{\pi^2 \nu^2}{3}\right) d\nu \,,
\label{eq:coherance}
\end{equation}
L'efficacité interférométrique dépend de trois termes : la bande
spectrale $\frac{\Delta\lambda}{\lambda_0}$, le taux de dilution de la
pupille $\frac{D'}{d'}$ et le déphasage $\Delta\phi_0$. Les deux
premiers paramètres sont à choisir lors de la conception de
l'instrument. Pour disposer d'une sensibilité optimale de
l'instrument, il est important d'avoir une cohérence $\mu$
maximale. Le choix du compromis entre bande passante et diamètre de
pupille de sortie peut être fait dans l'hypothése d'un déphasage nul
($\Delta \phi_0 =0$). Le facteur de cohérence s'écrit alors :
\begin{equation}
\mu \propto \int_\infty {\rm
sinc}\left(\frac{\Delta\lambda D'\pi}{\lambda_0 d'} \nu \right)
  \exp\left(-\frac{\pi^2 \nu^2}{3}\right) d\nu \,.
\end{equation}
La figure~\ref{fig:coher} représente $\mu$ en fonction du rapport
$\frac{\Delta\lambda D'}{\lambda_0 d'}$. Nous pouvons voir que plus
cette valeur est grande, plus la perte de cohérence est importante. Le
problème est d'aboutir à un compromis entre efficacité
interférométrique et largeur de bande spectrale. Le rapport signal sur
bruit optimum peut être un critére de choix. Dans le plan $u$-$v$, le
signal du pic frange est proportionnel à $\mu N_{\rm photons}$ alors
que le bruit de photons est proportionel à $\sqrt{N_{\rm photons}}$. En
considérant que $N_{\rm photons}$ est proportionel à la bande
spectrale, le signal sur bruit sera proportionel à $\mu
\sqrt{\Delta\lambda}$. La courbe correspondante est présentée dans la
partie droite de la figure~\ref{fig:coher}. Nous pouvons noter une
valeur optimum pour :
\begin{equation}
\frac{\Delta\lambda}{\lambda_0} =  1,15 \frac{d'}{D'}
\label{eq:delta_lam2}
\end{equation}
Cependant, il faut souligner que, dans un système à plusieurs fibres,
la distance $D'$ séparant deux sous-pupilles dépend de la paire de
fibres utilisée, et est donc variable.

{\bf Si l'on considére l'instrument dans son ensemble, on peut établir
  une relation entre la largeur de la bande passante et le diamètre de
  la pupille de sortie $\max(D'/d')$. Nous avons déduit de la
  relation~\ref{eq:delta_lam2} qu'une solution optimum peut être
  obtenue par:
\begin{equation}
\frac{\Delta\lambda}{\lambda_0} = 2 \frac{d'}{\max(D')}
\label{eq:delta_lambda}
\end{equation}
Il faut noter que lorsque $\frac{\Delta\lambda}{\lambda_0} >
\frac{d'}{D'}$ il existe un risque de confusion des fréquences
spatiales. Ceci doit être pris en compte lors du calcul de la
configuration non-redondante (voir section~\ref{sc:remap_chrom}).  }


\begin{figure}
   \centering
\resizebox{\hsize}{!}{
   \includegraphics{Images/coherence.eps}
   \includegraphics{Images/coherenceSB.eps}}
   \caption{ A gauche : efficacité interférométrique $\mu$ en fonction
   du rapport $\frac{\Delta\lambda D'}{\lambda_0 d'}$. Cette
   efficacité est supérieure à 0,5 pour une valeur de
   $\frac{\Delta\lambda D'}{\lambda_0 d'}$ inférieure à 2. A droite :
   l'efficacité interférométrique est multipliée par un terme
   proportionel à la racine carré de la bande passante. Pour une
   configuration donnée, ce graphique permet de choisir la bande
   passante optimisant le rapport signal sur bruit de photons.}
   \label{fig:coher}
\end{figure}


\subsection{Le champ interférométrique}
\label{sc:Champ_interfero}


\begin{figure}
   \centering
\resizebox{\hsize}{!}{
   \includegraphics{Images/Champ_inter.eps}}
   \caption{ Efficacité interférométrique en fonction de la bande
   spectrale et de la position de l'objet par rapport à l'axe
   optique. Une efficacité de 0,5 représente traditionnellement le
   champ de l'interféromètre. Cependant, lorsque l'on souhaite une
   mesure précise des visibilités d'un objet étendu, il est nécessaire
   d'avoir une efficacité interférométrique très stable entre les
   différentes bases. Une telle exigence est alors une contrainte
   très forte sur la bande passante. }
   \label{fig:champ_int}
\end{figure}

Le champ interférométrique, à la différence de celui de la fibre,
dépend de la bande spectrale et du ré-arrangement effectué.  Nous
avons représenté figure~\ref{fig:champ_int} l'efficacité en fonction
deux paramètres: la bande passante et le champ. Les courbes
correspondent à une perte d'efficacité de 0,1\%, 1\%, 10\% et 50\%.
Les courbes vertes sont tracées pour $D'/d'$ maximum, tel que
$\Delta\lambda/\lambda_0 = 2 d'/D'$. Les coubes rouges correspondent à
la situation la moins favorable, tel que $D'=2 d'$. La perte en
effacité interférométrique se situera pour une valeur comprise entre
les deux courbes.


Le champ interférométrique est communément défini par une efficacité
interférométrique telle que $\mu > 0,5$.  Il est parfois nécessaire de
décider d'une limite plus grande au champ afin d'éviter des écarts
d'efficacité entre les différentes bases. Il serait en effet
impossible de corriger ces variations a postériori et celles-ci
entraineraient des erreurs sur les visibilités obtenues. C'est
pourquoi il est donc préférable d'utiliser une bande passante adaptée
à la morphologie de l'objet. La figure~\ref{fig:champ_int} permet de
fixer la bande passante en fonction du champ et la précision demandée
sur les visibilités. Par exemple, pour un objet de largeur
$4\lambda/D$ et une précision souhaitée de 1\%, la bande passante
adaptée sera $\Delta\lambda/\lambda_0 \approx 0,022$. A l'opposé, si
l'objet observé est ponctuel avec, par exemple, un compagnon de très
faible intensité, on pourra revenir à une limitation du champ pour une
perte d'efficacité de 50\%.

Il est intéressant de comparer le champ de la fibre au champ
interférométrique. Ce dernier a été obtenu par la relation entre la
phase et le diamètre de la pupille d'entrée :
\begin{equation}
\Delta\phi_0=2\pi\alpha D/\lambda \,.
\label{ex:phi_alpha}
\end{equation}
C'est pourquoi la figure~\ref{fig:champ_int} représente le champ
interférométrique en fonction du facteur $\lambda/D$, au contraire de
la figure~\ref{fig:champ_fibre} qui représente celui de la fibre en
fonction de $\lambda/d$.  La conversion d'une abscisse à l'autre peut
s'opérer par le rapport $D/d$, une fois la pupille d'entrée
définie. 

Par ailleurs, en utilisant l'équation~\ref{eq:coherance} et~\ref{ex:phi_alpha},
nous obtenons l'écriture de l'efficacité interférométrique suivante :
\begin{equation}
\mu \propto \int_\infty {\rm
sinc}\left(\pi \frac{\Delta\lambda D'}{\lambda_0 d'}\left( \nu +
\frac{Dd'}{dD'} \alpha \left( \frac{d}{\lambda} \right)
\right)\right) \exp\left(-\frac{\pi^2 \nu^2}{3}\right) d\nu \,,
\end{equation} 
Cette expression met en exergue l'effet de proportionnalité entre le
champ interférométrique et le facteur ${Dd'}/{dD'}$. Elle nous fournit
un moyen de maximiser le champ lorsque l'on dispose les fibres dans la
pupille de sortie.

{\bf
Ainsi, il faut veiller, lors de la
reconfiguration de la pupille, à minimiser les rapports $\frac{Dd'}{dD'}$.
Par conséquent, nous chercherons à faire correspondre
les bases de la pupille d'entrée et de sortie de manière à ce que :
\begin{equation}
\sum_{\rm bases}{ \frac{Dd'}{dD'}}
\end{equation}
 soit minimum.
}



\subsection{Le bruit du piston atmosphérique}
\label{sc:piston}

\begin{figure}
   \centering
\resizebox{\hsize}{!}{
   \includegraphics{Images/Piston.eps}}
   \caption{ Effet de la bande passante et du piston atmosphérique sur
   l'efficacité interférométrique. Comme pour la
   figure~\ref{fig:champ_int}, les deux situations limites $D'/d = 2
   \lambda_0/\Delta\lambda$ et $D'/d' =2$ sont envisagées. Cette perte
   d'efficacité introduit un bruit sur la mesure des visibilités
   normalisées.  }
   \label{fig:piston}
\end{figure}

L'effet du piston atmosphérique peut également être déduit de
l'efficacité interférométrique.  La dimension de la pupille d'entrée,
ainsi que la longueur d'onde influent sur le déphasage ($\Delta
\phi_0$) provenant du piston. Par exemple, pour un piston de 3 $\mu$m
le déphasage donne $\Delta\phi_0 \approx 4\pi$ en bande H et
$\Delta\phi_0 \approx 9\pi$ dans le visible. A partir de
l'équation~\ref{eq:coherance}, nous avons pu déduire la perte
d'efficacité en fonction de la bande passante utilisée. Le
figure~\ref{fig:piston} donne ces résultats pour deux cas : $D'/d' =
2$ et $D'/d' = 2 \lambda_0/\Delta\lambda$. Comme nous l'avons vu dans
la section~\ref{sc:Champ_interfero}, ces deux situations permettent de
définir les conditions limites correspondant aux longueurs de base
maximales et minimales.

Nos résultats montrent que plus la bande spectrale est grande, plus
l'influence du piston atmosphérique sur les visibilités est
importante. Ainsi, pour un piston de 4 fois la longueur d'onde et une
bande spectrale de 0,02, l'erreur sur la visibilité sera de 1\%. Cette
erreur est multipliée par quatre pour une bande spectrale deux fois
plus faible. Il est important de noter qu'il s'agit d'un bruit
statistique, pouvant peut être diminué via plusieurs
observations. Cependant, les proprétés statistiques de la turbulence
rendent ce travail très difficile, et il ne faut pas s'attendre à une
diminution importante de l'erreur estimée par la
figure~\ref{fig:piston}.

%\subsection{Le bruit de piston atmosphérique}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Le choix du réarrangement}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Les contraintes du réarrangement}

Le réarrangement de pupille est une technique de codage de
l'information. Pour un processus d'imagerie classique, l'information
sur la turbulence et de l'objet astrophysique est mélangée. Pour
pouvoir distinguer les perubations instrumentales de l'information
astrophysique, il est necessaire de coder l'information manquante à
des fréquences supérieures.

La qualité de ce codage dépend du choix la configuration de la pupille
de sortie. Pour avoir une sensibilité maximale, il faut :
\begin{itemize}
\item utiliser un minimum de pixels, soit une plage minimale de
fréquences spatiales.
\item une bande spectrale la plus large possible, et par conséquent
  minimiser les rapports $D'/d'$ (équation~\ref{eq:delta_lambda}).
\end{itemize}
Or, le théorème de Shannon fixe le nombre de pixels nécessaire un à
bon échantillonage du plan fréquentiel par : $N_{\rm pixels} =
\max(D')/d'$. Ainsi, les deux conditions précédentes conduisent à
minimiser le rapport $\max(D')/d'$. Il faut déterminer la
configuration la plus compacte possible, tout en fournissant le moyen
de dissocier chacune des fréquences spatiales présentes. Cela
nécessite:
\begin{itemize}
\item un écart entre chaque fréquence présente d'au moins un
  pixel$^{-1}$, soit un $d'$.
\item une configuration non-redondante.
\end{itemize}
La première condition se traduit par la nécessité de disposer les
sous-pupilles sur une grille rectangulaire à maillage fixe de taille
$d'$. Le maillage optimum devant correspondre à 1 pixel$^{-1}$, il
doit être rectangulaire si les pixels le sont, et carré pour des
pixels carrés.  La seconde condition nécessite le développement d'un
algorithme spécifique.

Il faut également choisir entre une configuration non-redondante à une
dimension ou deux dimensions. Ce choix dépend de l'objectif
scientifique. Si l'on souhaite obtenir une
information spectrale de l'objet observé, il faut disperser les
franges, et pour cela disposer les fibres sur une seule
dimention. Dans le cas contraire, utiliser une configuration à
deux dimensions permet un arrangement plus compact.

\subsection{L'algorithme}

\begin{figure}[h]
   \centering
\resizebox{\hsize}{!}{
   \includegraphics{Images/Algorithm.eps}}
   \caption{Schéma de l'algorithme utilisé pour déterminer les
   configurations non-redondantes optimales. Elles sont toutes testés
   par l'utilisation d'une technique récursive.}
   \label{fig:algo}
\end{figure}

Si trouver une configuration non-redondante est aisé~\citep[par
exemple il existe des solutions proposées par][]{1970..Golay}, il est
autrement plus difficile de déterminer la configuration qui minimise la
valeur $\max(D')/d'$. Par exemple, un algorithme simple donnant une
configuration non-redondante fixe la position des
fibres de la façon suivante :
\begin{equation}
X_{(n)}=2^n d' \,.
\label{eq:algo_base}
\end{equation}
Un tel algorithme implique $\max(D')/d'=2^n$, une valeur loin d'être
optimale. Pour trouver les configurations optimales, nous avons
développé un algorithme de recherche de configurations
non-redondantes.  Le problème auquel nous avons tenté de résoudre est
le suivant : pour un rapport maximal $D'/d'$ donné, quel est le nombre
maximum de sous-pupilles placées sur une maille d'unités $d'$ qui
satisfont la propriété de non-redondance?


Cet algorithme a été programmé dans le langage Yorick. Il est schématisé
figure~\ref{fig:algo}.  Dans le cadre
d'une configuration redondante à une dimension, il est le suivant : \\
\texttt{
func Config(positions,positions\_libres,frequences,dimension,N\_but) \\
\{ \\
  N\_pos=dimsof(positions)(2); \\
  if (N\_pos >= N\_but) \\
    write,"N\_pos = "+pr1(N\_pos)+" ---
    Positions = "+pr1(positions);  \\
  for (i=positions(0)+1;i<=dimension;i++) \\
    if (positions\_libres(i))\\
      \{ \\
        frequences2=grow(frequences,i-positions); \\
        positions\_libres2=positions\_libres; \\
        positions\_libres2(frequences2*(frequences2 <=
	dimension-i)+i)=0; \\
        positions2=grow(positions,i); \\
        Config,positions2,positions\_libres2,frequences2,dimension,N\_but;\\
      \} \\
\} \\
}

Un des paramètres de la fonction est la variable
\texttt{N\_but}. Elle permet de préciser le nombre de
sous-pupilles que l'on cherche à disposer dans la grille. La fonction
se lance de la façon suivante : \\ \texttt{ dimension=18; \\
positions=[1]; \\ positions\_libres=array(short(1),dimension); \\
N\_but=6; \\
Config,positions,positions\_libres,frequences,dimension,N\_but; \\ }
On obtient au bout de quelques secondes : \\ \texttt{ N\_pos = 6 ---
Positions = [1,2,5,11,13,18] \\ N\_pos = 6 --- Positions =
[1,2,5,11,16,18] \\ N\_pos = 6 --- Positions = [1,2,9,12,14,18] \\
N\_pos = 6 --- Positions = [1,2,9,13,15,18] \\ N\_pos = 6 ---
Positions = [1,3,8,14,17,18] \\ N\_pos = 6 --- Positions =
[1,4,6,10,17,18] \\ N\_pos = 6 --- Positions = [1,5,7,10,17,18] \\
N\_pos = 6 --- Positions = [1,6,8,14,17,18] \\ }


Cet algorithme, récursif, a la propriété de calculer toutes les
possibilités de configurations non-redondantes. Il n'affiche un
résultat que si le nombre de fibres est supérieur à
\texttt{N\_but}. Par conséquent, le temps de réponse devient très long
lorsque le nombre de fibres dépasse $\approx 15$, mais la valeur
optimale au rapport $D'/d'$ est toujours fournie.  Dans le cadre d'une
configuration de la pupille à 2 dimensions nous nous sommes également
servi de cet algorithme. Pour cela, nous avons utilisé une maille à 2
dimensions, où un quart des emplacements sont disponibles, que nous
avons déplié sous la forme d'un tableau à une dimension. Il a ensuite
été fait appel à la fonction \texttt{Config} à l'instar d'une
configuration à une dimension.

\subsection{Configurations optimales}

\begin{figure}[h!]
   \centering
\resizebox{\hsize}{!}{
   \includegraphics{Images/Red1D.eps}}
   \caption{ Séries non-redondantes à une dimension. Ces
   configurations sont optimales car le plus compact possible. }
   \label{fig:red1d}
\end{figure}

\begin{figure}[h!]
   \centering
   \includegraphics[width=4.7cm]{Images/Red2D_2.eps}
\hfill
   \includegraphics[width=4.7cm]{Images/Red2D_3.eps}
\hfill
   \includegraphics[width=4.7cm]{Images/Red2D_4.eps} \vspace{.3cm}
\hfill
   \includegraphics[width=4.7cm]{Images/Red2D_5.eps}
\hfill
   \includegraphics[width=4.7cm]{Images/Red2D_6.eps}
\hfill
   \includegraphics[width=4.7cm]{Images/Red2D_7.eps} \vspace{.3cm}
\hfill
   \includegraphics[width=4.7cm]{Images/Red2D_8.eps}
\hfill
   \includegraphics[width=4.7cm]{Images/Red2D_9.eps}
\hfill
   \includegraphics[width=4.7cm]{Images/Red2D_10.eps} \vspace{.3cm}
\hfill
   \includegraphics[width=4.7cm]{Images/Red2D_11.eps}
\hfill
   \includegraphics[width=4.7cm]{Images/Red2D_12.eps}
\hfill
%   \includegraphics[width=5cm]{}
   \caption{ Séries non-redondantes à deux dimensions. Ces
   configurations sont optimales car le plus compact possible. }
   \label{fig:red2d}
\end{figure}

\begin{figure}[h!]
   \centering
   \includegraphics[width=7.cm]{Images/rearrangement1.eps}\hfill
   \includegraphics[width=7.cm]{Images/rearrangement2.eps}\vspace{.15cm}
   \includegraphics[width=7.cm]{Images/rearrangement3.eps}\hfill
   \includegraphics[width=7.cm]{Images/rearrangement4.eps}
   \caption{ En haut à gauche : Nombre de pixels par fibre en fonction
   du nombre de fibres. La courbe verte correspond à un réarrangement
   à 2 dimensions, et la rouge à un réarrangement à une dimension. Les
   courbes en pointillés resprésentent deux situations extrêmes où
   $N_{\rm Pixels}= N_{\rm Fibres} (N_{\rm Fibres-1})$ et ou $N_{\rm
   pixels}= 2^{N_{\rm Fibres}+1}$. En haut à droite : Base maximale en
   fonction du nombre de fibres. Dans le cas d'un réarrangement à une
   dimention, il s'agit de la longueur du tableau; dans celui à deux
   dimensions, il s'agit du diamètre du tableau. En bas : le rapport
   $N_{\rm Fibres}/N_{\rm Pixels} \times d'/\max(D')$ est proportionel au
   flux par pixel, alors que le rapport $1/(N_{\rm Fibres}-1) \times
   d'/\max(D')$ est proportionel au flux par fréquence spatiale. Ces
   deux valeurs traduisent la sensibilité de l'instrument au bruit de
   lecture et au bruit de photons. }
   \label{fig:rearrg}
\end{figure}

Les figures~\ref{fig:red1d} et~\ref{fig:red2d} représentent les
configurations les plus compactes possibles. Plus précisément, il est
impossible d'ajouter la présence d'une fibre dans chacun des
maillages. D'autres configurations non-redondantes ayant le même
nombre de fibres peuvent néanmoins exister. Les solutions obtenues
sont telles que, pour un nombre de fibres donné, le nombre de pixels
nécessaires pour respecter un bon échantillonage sera le mimimum. Ce
nombre de pixels est, d'après le théorème de Shannon, de $2
\max(D')/d'$ dans le cas d'un maillage à une dimension, et de $(2
\max(D')/d')^2 \pi/4$ pour d'un maillage à deux dimensions. Le rapport
$\pi/4$ provient du caractère circulaire de l'image de la fibre.

Le rapport du nombre de pixels sur celui des fibres est présenté dans
la figure~\ref{fig:rearrg} (haut-gauche). La courbe verte représente
le rapport dans le cadre d'un arrangement à 2 dimensions, et la courbe
rouge dans celui à une dimension. La première courbe en pointillés
donne les valeurs de codage limites tels que $\max(D')/d'=2^n$
(arlgorithme~\ref{eq:algo_base}) et $N_{\rm Pixels}=N_{\rm Fibres}
(N_{\rm Fibres}-1)$. La deuxième courbe correspond au minimum
théorique de codage où l'information sur chaque fréquence spatiale est
codée par 2 pixels. Nous nous en éloignons lorsque le nombre de fibres
augmente, la contrainte de non-redondance devenant plus forte.

Le rapport $N_{\rm Pixels}/N_{\rm Fibres}$ nous donne la répartition
du flux sur les pixels. Néanmoins, le rapport $D'/d'$ va également
conditionner le flux en limitant la bande spectrale utilisable. 
Nous avons établi section~\ref{sc:inf_spect} qu'il existe un optimum
en rapport signal sur bruit tel que : $\Delta\lambda/\lambda_0 = 2
d'/\max(D')$.  Ainsi, pour estimer une valeur proportionnelle au flux
par pixel, nous avons représenté sur la figure~\ref{fig:rearrg} le
rapport $N_{\rm Fibres}/ N_{\rm Pixels} \times d'/\max(D')$. Cette courbe
traduit la sensibilité de l'instrument au bruit de lecture et met
clairement en évidence l'avantage d'un ré-arrangement
non-redondant. De la même façon, si l'on remplace le nombre de pixels par
celui des fréquence spatiales, on abouti à une valeur qui
traduit la sensibilité de l'instrument au bruit de photons. Il
s'agit du rapport $1/(N_{\rm Fibres}-1) \times d'/\max(D')$.

Les deux graphiques du bas de la figure~\ref{fig:rearrg} montrent
l'intérêt, en terme de sensibilité au bruit de photons et du
détecteur, d'utiliser un réarrangement à deux dimensions. Cependant,
un certain nombre de pistes sont à explorer afin s'améliorer la
sensibilité :
\begin{itemize}
\item utiliser un détecteur à comptage de photons pour s'affranchir de
  la sensibilité au bruit de lecture.
\item faire interferer les fibres par groupes. Les conditions de déconvolution de
  l'algorithme section~\ref{sc:algo_eric} doivent néanmoins êtres respecté.
\item dans le cas d'un rearrangement à une dimension, disperser la
  lumière sur une bande spectrale la plus large possible. Le signal
  sur bruit par pixels n'en sera pas amélioré, mais ceci augmentera la
  limite en sensibilité due au bruit de photons.
\end{itemize}


\subsection{L'effet du chromatisme sur le codage fréquentiel}
\label{sc:remap_chrom}

\begin{figure}[h]
   \centering
   \includegraphics[width=7cm]{Images/frange_achro2.eps}\hfill
   \includegraphics[width=7cm]{Images/frange_chro.eps}
   \caption{ Effet du chromatisme sur le plan des fréquences
   spatiales. A gauche, les pics franges sont nettement définis sur
   l'image achromatique. A droite : le chromatisme (620 nm < $\lambda$
   < 640 nm) disperse les pics franges sur plusieurs fréquences
   spatiales.}
   \label{fig:chr_fr}
\end{figure}

Afin d'optimiser
la largeur de la bande passante, nous l'avons choisie celle-ci telle que
$\Delta\lambda/\lambda_0 = 2 d'/\max(D')$. Or, l'influence de la bande
passante va avoir pour effet d'élargir radialement le pic frange dans
le domaine de Fourier. Un exemple est donné figure~\ref{fig:chr_fr}
où le plan de Fourier est composé de 630 pics franges. L'image de
gauche correspond à un faisceau achromatique de longueur d'onde 630
nm et celle de droite à une bande passante entre 620 et 640
nm. Une confusion des pics franges est visible.

En l'abscence de déphasage, la fonction de modulation obtenue
(équation~\ref{eq:mod}) a une fréquence proportionnelle à
$1/D'\lambda$. Lorsque l'on prend en compte l'effet de la bande
passante, ces fréquences sont alors comprises entre
$1/D'(\lambda_0+\Delta\lambda/2)$ et
$1/D'(\lambda+\Delta\lambda/2)$. Ceci doit être intégré au calcul de
la configuration non-redondate de manière à ne pas poluer
l'information contenue aux différentes fréquences. Une modification de
l'algorithme à une dimention peut être faite en remplaçant la ligne 6
de l'algorithme par: \\ \texttt{ for
(i=positions(0)+1+max([0,$\frac{\lambda_0}{\Delta\lambda}$(dimension-i),$\frac{\lambda_0}{\Delta\lambda}$(i-1)])
;i<=dimension;i++) \\ }



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Le temps d'exposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
   \centering
   \includegraphics[width=7cm]{Images/S_B.eps}\hfill
   \includegraphics[width=7cm]{Images/S_B_F.eps}
   \caption{Signal sur bruit obtenu en fonction du temps
   d'observation et de la magnitude de l'objet observé, dans le cas
   d'un système à réarrangement de pupille composé de 36 fibres et
   fonctionnant dans le visible. A gauche : signal sur bruit par
   pixel. A droite : signal sur bruit par fréquence spatiale.}
   \label{fig:sb}
\end{figure}

Les trois paragraphes précédents nous ont permis de caractériser
l'instrument. Nous avons optimisé l'injection, la bande passante et
la géométrie du réarrangement. Lors d'une observation, il va être
nécessaire d'optimiser une dernier paramètre, celui du temps
d'exposition.

Comme pour toutes les techniques nécéssitant une déconvolution, le
réarrangement par fibres optiques suppose une turbulence fixe pendant
l'acquisition. Cette condition joue un rôle prépondérant sur la
qualité finale des données. Cependant, puisque la technique de codage
fréquentielle nécessite une dilution du flux de l'objet sur de
nombreux pixels, il faut optimiser le temps d'acquisition afin obtenir
un compromis entre le gel de la turbulence et le nombre de photons
reçu.

Nous avons fait ces calculs dans le cadre de l'instrument en projet à
l'observatoire. Il s'agit d'un système fibré à réarrangement de
pupille fonctionnant dans la longeur d'onde visible.  Le
paragraphe~\ref{sc:inject} fixe une taille de sous-pupilles de 3$r_0$
et un rapport d'ouverture entre la fibre et les lentilles $\eta
=1,5$. L'efficacité de couplage est alors en moyenne $\rho=10\%$. La
pupille de sortie choisie est une configuration non-redondante en deux
dimensions de rapport $\max(D'/d') = 40$. Le nombre du pixels utilisé
sera par conséquent d'approximativement $N_{\rm pixels} =
5\,000$. Enfin, nous avons choisi d'optimiser la bande passante en
fonction de l'équation~\ref{eq:delta_lambda}, ce qui nous donne
$\Delta\lambda/\lambda_0=0.05$ pour une efficacité interférométrique
moyenne de $\mu = 0,75$. En ne considérant que le bruit de photons,
nous pouvons en déduire un rapport signal sur bruit par pixel :
\begin{equation}
S/B_{\rm pixel}=\mu \sqrt{\frac{N_{\rm photons}}{N_{\rm pixels}} \rho
  \Delta\lambda Q t} 
\end{equation}
ainsi qu'un signal sur bruit par fréquence spatiale :
\begin{equation}
S/B_{\rm fréquence}=\mu \sqrt{\frac{N_{\rm photons}}{N_{\rm Fibres} (N_{\rm Fibres}-1)} \rho
  \Delta\lambda Q t} 
\end{equation}
où $N_{\rm photons}$ est le nombre de photons par sous-pupille et par
unité de longueur d'onde, $Q$ l'efficacité quantique du détecteur et
$t$ le temps d'intégration par pose. En considérant une caméra à
comptage de photons, fonctionnant dans le visible ($Q=0,2$), la courbe
de gauche de la figure~\ref{fig:sb} nous donne le signal sur bruit
obtenu par pixel en fonction du temps d'observation. Si le détecteur
présente un bruit de lecture, la sensibilité de l'instrument serait
très faible. Dans le cadre d'un instrument infrarouge par exemple, il
serait necessaire de restreindre le nombre de fibres à recombiner
simultanément. En l'abscence de bruit de lecture, le signal sur bruit
par fréquence spatiale fixe la sensibilité de l'instrument. Nous avons
montré Chapitre 3 que notre algorithme permet le traitement de
fréquence spatiales ayant un signal sur bruit aux environs de 0,1. Il
est par conséquent nécessaire de choisir le temps de pose pour que le
signal sur bruit soit au minimum égal à cette valeur.


==> titlepage.tex <==
%\setlength{\unitlength}{1cm}
%\begin{picture}
%\put(20,25){
%\enlargethispage{1cm}

\thispagestyle{empty}
\def\cnt#1{\begin{center}{#1}\end{center}}


%\large\vspace*{-1cm}
%\cnt{\Large\sffamily ISAS}%
%\vspace{-.7cm}
%\cnt{\Large\sffamily Universit\`a degli studi di Pisa}%
%\vspace{-.7cm}
%\cnt{\Large\sffamily FOR ADVANCED STUDIES}%
\vskip 2.5cm

\cnt{\large\bf Doctorat de l'universit\'e Paris 6}
\vskip 1cm
\cnt{\Large\sffamily Ann\'ees universitaires 2003-2006}
\vskip 3cm
\cnt{\Huge\bf Imagerie des étoiles évoluées  }
\cnt{\Huge\bf par interférométrie  }
\vskip 5cm
\cnt{\Large \bf Sylvestre Lacour}
\cnt{\Large sous la direction de}
\cnt{\Large \bf Guy Perrin}
\cnt{\Large \`a l'observatoire de paris Meudon}


%\end{picture}










